FedAvg with Fine Tuning: Local Updates Lead to Representation Learning

The Federated Averaging (FedAvg) algorithm, which consists of alternating between a few local stochastic gradient updates at client nodes, followed by a model averaging update at the server, is perhaps the most commonly used method in Federated Learning. Notwithstanding its simplicity, several empirical studies have illustrated that the output model of FedAvg, after a few fine-tuning steps, leads to a model that generalizes well to new unseen tasks. This surprising performance of such a simple method, however, is not fully understood from a theoretical point of view. In this paper, we formally investigate this phenomenon in the multi-task linear representation setting. We show that the reason behind generalizability of the FedAvg's output is its power in learning the common data representation among the clients' tasks, by leveraging the diversity among client data distributions via local updates. We formally establish the iteration complexity required by the clients for proving such result in the setting where the underlying shared representation is a linear map. To the best of our knowledge, this is the first such result for any setting. We also provide empirical evidence demonstrating FedAvg's representation learning ability in federated image classification with heterogeneous data.

==> App_Finite.tex <==
\section{Finite-Sample Case}

\subsection{Concentration lemmas}

\begin{lemma} \label{lem:concen1}
Let $\mathbf{\Sigma}\coloneqq \frac{1}{b} \sum_{j=1}^b \mathbf{x}_j \mathbf{x}_j^\top$ be the empirical gram matrix formed by $b$ samples from a mean-zero, $\mathbf{I}_d$-sub-gaussian distribution. 
Let $\mathbf{U}\in \mathbb{R}^{d \times d_1}$ and $\mathbf{V}\in\mathbb{R}^{d \times d_2}$ be two matrices independent of the randomness in $\mathbf{\Sigma}$.
Then for any $\gamma: 0 <\gamma< c (b - d_1 - d_2)$ and absolute constants $c,c',c''$,
\begin{align}
    \|\mathbf{U}^\top \mathbf{{\Sigma}}\mathbf{V} - \mathbf{U}^\top \mathbf{V}\|_2\leq c' \|\mathbf{U}\|\|\mathbf{V}\|\frac{\sqrt{d_1+d_2} +{\gamma}}{\sqrt{b}}
\end{align}
with probability at least $1-\exp(c''\gamma^2)$.
\end{lemma}

\begin{proof}
The proof follows by  sub-exponential concentration combined with an $\epsilon$-net argument as in the proof of Theorem 4.6.1. in \cite{vershynin2018high}. 
First note that \begin{align}\| \mathbf{U}^\top \mathbf{{\Sigma}}\mathbf{V} - \mathbf{U}^\top \mathbf{V}\|_2 = \sup_{\mathbf{\bar{w}}_1 \in \mathcal{S}^{d_1-1},\mathbf{\bar{w}}_2 \in \mathcal{S}^{d_2-1}}  \bigg|  \tfrac{1}{b}  \sum_{j=1}^b\mathbf{\bar{w}}_1^\top \mathbf{U}^\top  \mathbf{x}_j\mathbf{x}_j^\top\mathbf{V} \mathbf{\bar{w}}_2   - \mathbf{\bar{w}}_1^\top\mathbf{U}^\top \mathbf{V} \mathbf{\bar{w}}_2   \bigg| \end{align}

Let $\mathcal{M}_1$ be an $\tfrac{\epsilon}{4}$-net over $\mathcal{S}^{d_1 - 1} \coloneqq \{ \mathbf{w}_1\in\mathbb{R}^{d_1}: \|\mathbf{w}_1\| = 1 \}$ and let $\mathcal{M}_2$ be an $\tfrac{\epsilon}{4}$-net over $\mathcal{S}^{d_2 - 1} \coloneqq \{ \mathbf{w}_2\in\mathbb{R}^{d_2}: \|\mathbf{w}_2\| = 1 \}$. By Corollary 4.2.13 in \cite{vershynin2018high}, we have that such nets exist with at most $9^{d_1}$ and $9^{d_2}$ elements, respectively.

Consider any fixed $\mathbf{w}_1\in \mathcal{M}_1$ and $\mathbf{w}_2 \in \mathcal{M}_{2}$. By the $\mathbf{I}_d$-sub-gaussianity of $\mathbf{x}_j$, the random variable
$\mathbf{w}_1^\top \mathbf{U}^\top \mathbf{x}_j\mathbf{x}_j^\top \mathbf{V} \mathbf{w}_2  - \mathbf{w}_1^\top\mathbf{U}^\top \mathbf{V} \mathbf{w}_2$ is sub-exponential with mean zero and variance proxy $c\|\mathbf{U}\|\|\mathbf{V}\|$, independently for each $j$. 
Thus, by Bernstein’s Inequality, for any $\gamma > 0, (\sqrt{d_1+d_2} + \gamma)^2 \leq b$ and an absolute constant $c$,
\begin{align}
\mathbb{P}\bigg( \bigg| \frac{1}{b}  \sum_{j=1}^b  &\mathbf{w}_1^\top \mathbf{U}^\top \mathbf{x}_j\mathbf{x}_j^\top \mathbf{V} \mathbf{w}_2  - \mathbf{w}_1^\top\mathbf{U}^\top \mathbf{V} \mathbf{w}_2   \bigg| <  \|\mathbf{U}\|\|\mathbf{V}\|\tfrac{\sqrt{d_1+d_2} + \gamma}{\sqrt{b}} \bigg) \nonumber \\
&\geq  1 - 2 \exp\bigg( - cb\min \bigg(  \tfrac{\sqrt{d_1+ d_2} + \gamma}{\sqrt{b}}, \bigg(\tfrac{\sqrt{d_1+ d_2} + \gamma}{\sqrt{b}}\bigg)^2 \bigg) \bigg)\nonumber \\
&\geq 1 - 2 \exp\big( - c' (d_1+d_2 + \gamma^2) \big)
\end{align} 
where $\delta =  \tfrac{\sqrt{d_1+ d_2} + \gamma}{\sqrt{b}}$ and the second inequality follows since $b \geq (\sqrt{d_1+d_2} + \gamma)^2$.
Union bounding over all $\mathbf{w}_1 \in \mathcal{M}_1$ and $\mathbf{w}_2 \in \mathcal{M}_2$ yields
\begin{align}
\mathbb{P}\bigg( \max_{\mathbf{w}_1 \in \mathcal{M}_1,\mathbf{w}_2 \in \mathcal{M}_2} &\bigg| \tfrac{1}{b}  \sum_{j=1}^b  \mathbf{w}_1^\top \mathbf{U}^\top \mathbf{x}_j\mathbf{x}_j^\top \mathbf{V} \mathbf{w}_2  - \mathbf{w}_1^\top\mathbf{U}^\top \mathbf{V} \mathbf{w}_2   \bigg| <  \|\mathbf{U}\|\|\mathbf{V}\|\tfrac{\sqrt{d_1+d_2} + \gamma}{\sqrt{b}} \bigg) \nonumber \\ &\geq  1 - 2 \times 9^{d_1+d_2} \exp\big( - c' (d_1+d_2 + \gamma^2) \big)\nonumber \\
 &\geq 1 - 2\exp\big( - c'  \gamma^2 \big) \nonumber
\end{align} 
for a sufficiently large constant $c'$. 
Finally, since any $\mathbf{\bar{w}}_1 \in \mathcal{S}^{d_1-1}$ and $\mathbf{\bar{w}}_2 \in \mathcal{S}^{d_2-1}$ are each $\tfrac{\epsilon}{4}$-close in Euclidean distance to some $\mathbf{w}_1\in \mathcal{M}_1$ and $\mathbf{w}_2 \in \mathcal{M}_{2}$, respectively, we have 
\begin{align}
\mathbb{P}\bigg(& \sup_{\mathbf{\bar{w}}_1 \in \mathcal{S}^{d_1-1},\mathbf{\bar{w}}_2 \in \mathcal{S}^{d_2-1}} \bigg| \tfrac{1}{b}  \sum_{j=1}^b  \mathbf{\bar{w}}_1^\top \mathbf{U}^\top \mathbf{x}_j\mathbf{x}_j^\top \mathbf{V} \mathbf{\bar{w}}_2  - \mathbf{\bar{w}}_1^\top\mathbf{U}^\top \mathbf{V} \mathbf{\bar{w}}_2   \bigg| \geq   \|\mathbf{U}\|\|\mathbf{V}\|\tfrac{\sqrt{d_1+d_2} + \gamma}{\sqrt{b}} \bigg) \nonumber \\
&\leq 2 \mathbb{P}\bigg(\max_{\mathbf{w}_1 \in \mathcal{M}_1,\mathbf{w}_2 \in \mathcal{M}_2} \bigg| \tfrac{1}{b}  \sum_{j=1}^b  \mathbf{w}_1^\top \mathbf{U}^\top \mathbf{x}_j\mathbf{x}_j^\top \mathbf{V} \mathbf{w}_2  - \mathbf{w}_1^\top\mathbf{U}^\top \mathbf{V} \mathbf{w}_2   \bigg| <   \|\mathbf{U}\|\|\mathbf{V}\|\tfrac{\sqrt{d_1+d_2} + \gamma}{\sqrt{b}} \bigg) \nonumber 
\end{align}
thus 
\begin{align}
\mathbb{P}\bigg(& \sup_{\mathbf{\bar{w}}_1 \in \mathcal{S}^{d_1-1},\mathbf{\bar{w}}_2 \in \mathcal{S}^{d_2-1}}  \bigg| \tfrac{1}{b}  \sum_{j=1}^b  \mathbf{\bar{w}}_1^\top \mathbf{U}^\top \mathbf{x}_j\mathbf{x}_j^\top \mathbf{V} \mathbf{\bar{w}}_2  - \mathbf{\bar{w}}_1^\top\mathbf{U}^\top \mathbf{V} \mathbf{\bar{w}}_2   \bigg| \geq   \|\mathbf{U}\|\|\mathbf{V}\|\tfrac{\sqrt{d_1+d_2} + \gamma}{\sqrt{b}} \bigg) \nonumber \\
&\geq 1 - 4 \exp\big( - c'  \gamma^2 \big) \nonumber 
\end{align}
as desired.
\end{proof}


\begin{lemma}\label{lem:concen2}
Let $\mathbf{\Sigma}\coloneqq \frac{1}{b}\sum_{j=1}^b \mathbf{x}_j \mathbf{x}_j^\top$ be the empirical gram matrix formed by $b$ samples from a mean-zero, $\mathbf{I}_d$-sub-gaussian distribution. 
Let $\mathbf{U}\in \mathbb{R}^{d \times d_1}$ and $\mathbf{V}\in\mathbb{R}^{d \times d_2}$ be two matrices independent of the randomness in $\mathbf{\Sigma}$.
Then for any $\gamma: 0 <\gamma< c (Mb - d_1 - d_2)$ and absolute constants $c,c',c''$,
\begin{align}
    \left\|\frac{1}{M}\sum_{i=1}^M \mathbf{U}_i^\top \mathbf{{\Sigma}}\mathbf{V}_i - \mathbf{U}_i^\top \mathbf{V}_i\right\|_2\leq c'\max_{i\in [M]}\{\|\mathbf{U}_i\|\|\mathbf{V}_i\|\}\frac{\sqrt{d_1+d_2} +{\gamma}}{\sqrt{M b}}
\end{align}
with probability at least $1-\exp(c''\gamma^2)$.
\end{lemma}

\begin{proof}
The argument is analogous to that in in Lemma \ref{lem:concen1} but with $Mb$ independent sub-exponential random variables rather than $b$, and each with maximum sub-exponential variance proxy $c \max_{i \in [M]} \|\mathbf{U}_i\|\|\mathbf{V}_i\|$.
\end{proof}


\begin{lemma}\label{lem:concen3}
Let $\mathbf{\Sigma}$ be the empirical covariance formed by $b$ samples from a mean-zero, $\mathbf{I}_d$-sub-gaussian distribution. 
Let $\mathbf{U}\in \mathbb{R}^{d \times d_1}$ and $\mathbf{V}\in\mathbb{R}^{d \times d_2}$ be two matrices independent of the randomness in $\mathbf{\Sigma}$.
Then for any $\gamma: 0 <\gamma< c (Mb - d_1 - d_2)$ and absolute constants $c,c',c''$,
\begin{align}
    \left\|\frac{1}{M}\sum_{i=1}^M \mathbf{U}_i^\top \mathbf{{\Sigma}}\mathbf{V}_i - \mathbf{U}_i^\top \mathbf{V}_i\right\|_2\leq c'\max_{i\in [M]}\{\|\mathbf{U}_i\|\|\mathbf{V}_i\|\}\frac{\sqrt{d_1+d_2} +{\gamma}}{\sqrt{M b}}
\end{align}
with probability at least $1-\exp(c''\gamma^2)$.
\end{lemma}

\begin{proof}
The argument is analogous to that in in Lemma \ref{lem:concen1} but with $Mb$ independent sub-exponential random variables rather than $b$, and each with maximum sub-exponential variance proxy $c \max_{i \in [M]} \|\mathbf{U}_i\|\|\mathbf{V}_i\|$.
\end{proof}



% \begin{proposition}

% \end{proposition}

% \begin{proof}

% \end{proof}

% \begin{lemma}
% Sum of size-$b$ subset of sub-exponential random variables is close to ambient mean (for a fixed U V)
% \end{lemma}

% \begin{proof}

% \end{proof}

% \begin{lemma}
% covariance of subset is close to covariance of set for a fixed U V
% \end{lemma}

% \begin{proof}

% \end{proof}

% \begin{lemma}
% covariance of set is close to effective identity for a fixed U, V
% \end{lemma}

% \begin{proof}

% \end{proof}

\begin{lemma}
concentration holds for all k-dim instances in the algorithm execution
\end{lemma}

\begin{proof}
take union bound, add an extra $\log(\tau \log(1\epsilon))$ factor to the batch complexity
\end{proof}


\subsection{Representation learning proofs}

Table of notations.

\begin{table}[h]
\begin{tabular}{|c|l|}
\hline
\textbf{Notation}                                                                                                                                & \textbf{Definition}                                \\ \hline
$\del_t$                                                    & $\mathbf{I}_k - \alpha \mathbf{B}_t^\top \mathbf{B}_t$                        \\ 
$\deld_t$                & $\mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top$ \\ 
$L_\ast$                                                                                      & $\max_{t\in [T]} \sigma_{\max}^{0.5}\left(\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\right)\leq L_\ast$ almost surely  \\ 
$\mu_\ast$                                                                                      & $0< \mu_\ast \leq \min_{t\in [T]} \sigma_{\min}^{0.5}\left(\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\right)$  almost surely \\
$\eta_\ast$                                                                                      & $\max_{t\in [T]} \left\|\tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\right\|_2 \leq \eta_\ast \leq L_\ast$ almost surely  \\
$L_{\max}$                                                                                      & $\max_{t\in [T],i\in[n]}\|\mathbf{w}_{\ast,t,i}\|_2 \leq L_{\max}\leq c\sqrt{k} L_\ast$ almost surely for constant $c$ \\ 
%  $\sigma$       & Noise variance \\ 
$\kappa_\ast$                                                                                      & $\nicefrac{L_\ast}{\mu_\ast}$  \\ 
$\kappa_{\ast,\max}$                                                                                      & $\nicefrac{L_{\max}}{\mu_\ast}$  \\ 
$\boldsymbol{\delta}_{t,i,s}$ & $\coloneqq \mathbf{I}_k - \alpha\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top $, i.e. the product error for the $s$-th local iteration for task $i$ at round $t$ \\
$\mathbf{e}_{t,i,s}$ & $\coloneqq \mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i} $, i.e. the product error for the $s$-th local iteration for task $i$ at round $t$ \\
% $\mathbf{\Sigma}_{t,i}$ & $\coloneqq \tfrac{1}{n_i}\sum_{j=1}^{n_i}\mathbf{x}_{t,i,j}\mathbf{x}_{t,i,j}^\top$ \\
$\mathbf{X}_{t,i,s}$ &  $\coloneqq [\mathbf{x}_{t,i,s,j}^\top]_{j\in [b]} \in \mathbb{R}^{m \times d}$, i.e. the matrix of data vectors at update $(t,i,s)$  \\
$\mathbf{{\Sigma}}_{t,i,s}$ & $\coloneqq \tfrac{1}{b}\sum_{j=1}^{b}\mathbf{x}_{t,i,s,j}\mathbf{x}_{t,i,s,j}^\top$, i.e. the empirical covariance for the $s$-th local iteration for task $i$ at round $t$ \\
$\mathbf{z}_{t,i,s}$ & $\coloneqq [z_{t,i,s,j}]_{j\in [b]} \in \mathbb{R}^{b}$, i.e. the vector of noise values for the batch at update $(t,i,s)$ \\
\hline
\end{tabular}
\end{table}




\begin{proof}
% \begin{enumerate}
% \item $A_1(t) \coloneqq \{ \|\mathbf{w}_t - \alpha \mathbf{B}_{t-1}^\top\mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t-1}\|_2 \leq   \alpha^{2.5}\kappa_\ast^2 L_\ast^2 \eta_\ast \}$
%     \item {$A_2(t) \coloneqq \{ \|\mathbf{w}_t \|_2 \leq   c_2 \sqrt{\alpha} \eta_\ast \}$}
%     % \item $A_3(t) \coloneqq \{ \|\del_t \|_2 \leq  (1 - 0.5 \alpha^2 \mu_\ast^2 E_0)\|\del_{t-1} \|_2 + c_3 \alpha^4 L_\ast^4 \}$
%     \item $A_3(t) \coloneqq \{ \|\del_t \|_2 \leq  c_3 \alpha^2 \kappa_\ast^2 L_\ast^2 \}$
%     \item $A_4(t) \coloneqq \{ \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_t\|_2 \leq  (1 - 0.5 \alpha^2 \mu_\ast^2 E_0)\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t-1} \|_2  \}$
%     \item $A_5(t) \coloneqq \{ \dist_t \leq  (1 - 0.5 \alpha^2 \mu_\ast^2 E_0)\dist_{t-1}  \}$
% \end{enumerate}
% \begin{enumerate}
%     \item 
% \end{enumerate}
\begin{enumerate}
    \item $A_{1,t,i}(s) \coloneqq \{\|\mathbf{w}_{t,i,s'}- \alpha \mathbf{B}_{t,i,s'-1}^\top \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}\|_2 \leq c_1'\alpha^{2.5} \tau  L_{\max}^3  \kappa_{\max}^2 \quad \forall s'\in \{1,\dots,s\}\}$
    
     \item $A_{2,t,i}(s) \coloneqq \{\|\del_{t,i,s'}\|_2 \leq c_2'\alpha^2 L_\ast^2 \kappa_{\max}^2(1 + \tfrac{\sqrt{k} + \sqrt{\log(M\tau)}}{\sqrt{n_i}}) \quad \forall s'\in \{1,\dots,s\}  \}$ 
    
%O(\|\del_{t,i,s-1}\|_2 \|\mathbf{w}_{t,i,s-1}\|_2)\equiv

        % \item $A_{3,t,i}(s)\coloneqq \{\|\mathbf{e}_{t,i,s}\|_2 \leq (1 - c_3\alpha^2\|\mathbf{w}_{\ast,t,i}\|_2^2)\|\mathbf{e}_{t,i,s-1}\|_2\}$
        
        \item $A_{3,t,i}(s)\coloneqq \{ \dist(\mathbf{B}_{t,i,s'}, \mathbf{B}_\ast) \leq 2  \dist(\mathbf{B}_{t}, \mathbf{B}_\ast)\quad \forall s'\in \{1,\dots,s\}\}$
        
        % , where $\mathbf{q}_{t,i,s}\coloneqq \mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}$.
    \end{enumerate}
The second set of inductions controls the global behavior, starting from $t=1$ as the base case:
\begin{enumerate}
\item $A_1(t) \coloneqq \{ \|\mathbf{w}_{t'} - \alpha(\mathbf{I}_k + \del_{t'}) \mathbf{B}_{t'}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t'}\|_2 \leq   \alpha^{2.5}\tau L_{\max}^3 + c \alpha^{4.5}\tau^2 L_{\max} c_{\del}^2 \quad \forall t'\in \{1,\dots, t\}\}$ % means that we'll need alpha leq kappa2
% \alpha^{2.5}\kappa_\ast^2 L_\ast^2 \eta_\ast \}$
    % \item {$A_2(t) \coloneqq \{ \|\mathbf{w}_t \|_2 \leq   c_2 \sqrt{\alpha} \eta_\ast \}$}
    % \item $A_3(t) \coloneqq \{ \|\del_t \|_2 \leq  (1 - 0.5 \alpha^2 \mu_\ast^2 E_0)\|\del_{t-1} \|_2 + c_3 \alpha^4 L_\ast^4 \}$
    \item $A_2(t) \coloneqq \{ \|\del_{t'} \|_2 \leq  c_3 \alpha^2 \tau  L_{\max}^2  \kappa_{\max}^2 \quad \forall t'\in \{1,\dots, t\}\}$
    \item $A_3(t) \coloneqq \{ \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t'}\|_2 \leq  (1 - 0.4 \alpha^2 \mu_\ast^2 E_0)\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t'-1} \|_2 \quad \forall t'\in \{1,\dots, t\} \}$
    \item $A_4(t) \coloneqq \{ \dist_{t} \leq  (1 - 0.4 \alpha^2 \mu_\ast^2 E_0)^{t-1} \quad \forall t'\in \{1,\dots, t\}  \}$
\end{enumerate}

\end{proof}





\begin{lemma}[$A_{1,t,i}(s+1)$] \label{lem:la1s} 

\begin{align}
    \|\mathbf{w}_{t,i,s+1} -  \alpha \mathbf{B}_{t,i,s}\mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \| &\leq c' \alpha^{2.5} \tau L_{\max}^3 \kappa_{\max}^2 + c \alpha^{0.5}(L_{\max}+\sigma)
\end{align}

\end{lemma}

\begin{proof}
Since $\mathbf{w}_{t,i,s+1} = \del_{t,i,s-1}\mathbf{w}_{t,i,s-1} + \alpha \mathbf{B}_{t,i,s-1}\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}$,  
 \begin{align}
    \| \mathbf{w}_{t,i,s+1} -  \alpha \mathbf{B}_{t,i,s}\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}  &=\|\del_{t,i,s-1}\mathbf{w}_{t,i,s-1} \|_2 \nonumber \\
     &\leq c \alpha^3 \tau L_{\max}^2 \kappa_{\max}^2 \|\mathbf{B}_{t,i,s-2}^\top\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\|_2\nonumber \\
     &\leq  c' \alpha^{2.5} \tau L_{\max}^3 \kappa_{\max}^2 
 \end{align}
by  $A_{1,t,i}(s)$ and $A_{2,t,i}(s)$.
\end{proof}

\begin{lemma}[$A_{2,t,i}(s+1)$]

\end{lemma}

\begin{proof}
    %  Let $\del_{t,i,s}\coloneqq \mathbf{I}_k - \alpha \mathbf{B}_{t,i,s}^\top\mathbf{B}_{t,i,s}$. Then $\|\del_{t,i,s}\|_2 \leq c_2\|\del_t\|_2 \leq c_2'\alpha^2 L_\ast^2 \kappa_\ast^2$ where $c_2>1$.
    % Let $\mathbf{e}_{t,i,s}\coloneqq \mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$ and  $\mathbf{G}_{t,i,s} \coloneqq \mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}$.
   We argue similarly as in Lemma \ref{lem:a2s}. Let $\mathbf{\hat{G}}_{t,i,s} \coloneqq \tfrac{1}{\alpha}(\mathbf{B}_{t,i,s} - \mathbf{B}_{t,i,s+1})= \mathbf{\Sigma}_{t,i,s} \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top + \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top$ and 
    $\mathbf{N}_{t,i,s} \coloneqq \mathbf{G}_{t,i,s}-\mathbf{\hat{G}}_{t,i,s} = (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top - \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top$.
    We have 
    \begin{align}
        \del_{t,i,s+1} &= \del_{t,i,s}  + \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{\hat{G}}_{t,i,s} +\alpha^2 \mathbf{\hat{G}}_{t,i,s}^\top \mathbf{B}_{t,i,s} - \alpha^3 \mathbf{\hat{G}}_{t,i,s}^\top \mathbf{\hat{G}}_{t,i,s} \nonumber \\  %\\
        &= \del_{t,i,s}  + \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{{G}}_{t,i,s} +\alpha^2 \mathbf{{G}}_{t,i,s}^\top \mathbf{B}_{t,i,s} - \alpha^3 \mathbf{{G}}_{t,i,s}^\top \mathbf{{G}}_{t,i,s} \nonumber \\
        &\quad - \alpha^2 \mathbf{{B}}_{t,i,s}^\top \mathbf{N}_{t,i,s} - \alpha^2 \mathbf{N}_{t,i,s}^\top\mathbf{{B}}_{t,i,s}  - \alpha^3 \mathbf{N}_{t,i,s}^\top \mathbf{G}_{t,i,s} +\alpha^3 \mathbf{\hat{G}}_{t,i,s}^\top \mathbf{N}_{t,i,s}
        % &= \del_{t,i,s}  + \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{{G}}_{t,i,s} +\alpha^2 \mathbf{{G}}_{t,i,s}^\top \mathbf{B}_{t,i,s} - \alpha^3 \mathbf{{G}}_{t,i,s}^\top \mathbf{{G}}_{t,i,s} \nonumber  \\
        % &\quad - \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{{N}}_{t,i,s} -\alpha^2 \mathbf{{N}}_{t,i,s}^\top \mathbf{B}_{t,i,s} + \alpha^3 \mathbf{{G}}_{t,i,s}^\top \mathbf{{N}}_{t,i,s} + \alpha^3 \mathbf{{N}}_{t,i,s}^\top \mathbf{\hat{G}}_{t,i,s} 
    \end{align}
    % By the same analysis as in Lemma \ref{lem:a2s}, we know that
    % \begin{align}
    %     \| \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{{G}}_{t,i,s} +\alpha^2 \mathbf{{G}}_{t,i,s}^\top \mathbf{B}_{t,i,s} - \alpha^3 \mathbf{{G}}_{t,i,s}^\top \mathbf{{G}}_{t,i,s}\|&= \mathcal{O}(\alpha^4 \tau^2 L_{\max}^4) \nonumber 
    % \end{align}
    % We also know that by Lemma \ref{lem:concen1},
    % \begin{align}
    %     \|
    % \end{align}
    Note that 
    \begin{align}
       \| \mathbf{{B}}_{t,i,s}^\top \mathbf{N}_{t,i,s}\| &= \|\mathbf{{B}}_{t,i,s}^\top(\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top - \tfrac{1}{b}\mathbf{{B}}_{t,i,s}^\top\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top\|\nonumber \\
       &\leq \|\mathbf{{B}}_{t,i,s}^\top(\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top\| + \|\tfrac{1}{b}\mathbf{{B}}_{t,i,s}^\top\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top\|\nonumber \\
       &\leq c L_{\max}(L_{\max} +\sigma) \tfrac{\sqrt{k} + \gamma }{\sqrt{b}}  \label{hp}
    \end{align}
    where \eqref{hp} follows with probability at least $1 - c e^{-c' \gamma^2}$ for any $\gamma: 0< \gamma < b - k -1$ by Lemma \ref{lem:concen1}. 
    Similarly, 
    \begin{align}
        \|\mathbf{N}_{t,i,s}^\top \mathbf{G}_{t,i,s} \| &\leq \|((\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top - \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top)^\top \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top \| \nonumber \\
        &\leq  |\langle \mathbf{e}_{t,i,s}, (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\rangle|  \|\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top\| +  |\langle  \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s} , \mathbf{e}_{t,i,s} \rangle| \|\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top\| \nonumber \\
        &\leq c \alpha L_{\max}^3(L_{\max}+\sigma)\tfrac{1 + \gamma}{\sqrt{b}} \nonumber
    \end{align}
    with probability at least $1- c e^{-c' \gamma^2}$. Lastly, we have
    \begin{align}
      \|&\mathbf{\hat{G}}_{t,i,s}^\top \mathbf{N}_{t,i,s}\| \nonumber \\
      &=  \|( \mathbf{\Sigma}_{t,i,s}\mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top  +  \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top)^\top((\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top - \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top) \|    \nonumber   \\
      &\leq |\langle \mathbf{\Sigma}_{t,i,s} \mathbf{e}_{t,i,s}, (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\rangle| \|\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top\| \nonumber \\
      &\quad + | \langle \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s},  (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\rangle | \|\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top\| \nonumber \\
      &\quad +  | \langle \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s},  \mathbf{\Sigma}_{t,i,s} \mathbf{e}_{t,i,s}\rangle | \|\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top\| \nonumber \\
      &\quad +  | \langle \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s},  \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\rangle | \|\mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top\|  \nonumber \\
      &\leq     \label{hhh}
    %   \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top)^\top
    %   ((\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top - \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top) \|  
    \end{align}
    where \eqref{hhh} follows with probability at least $ 1- c\exp ()$ by Lemma \ref{lem:concen3}. 
    
    ---
    
    Next, by Lemma \ref{lem:a2s}, we have almost surely
    \begin{align}
        \|\del_{t,i,s}  + \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{\hat{G}}_{t,i,s} +\alpha^2 \mathbf{{G}}_{t,i,s}^\top \mathbf{B}_{t,i,s} - \alpha^3 \mathbf{{G}}_{t,i,s}^\top \mathbf{{G}}_{t,i,s}\| &\leq \|\del_{t,i,s}\| + O(\alpha^4 \tau L_{\max}^4) \nonumber
    \end{align}
    

    
    which means that 
    \begin{align}
        \|\del_{t,i,s+1}\|_2 &\leq \|\del_{t,i,s}\| + O(\alpha^4 \tau L_{\max}^4 + \alpha^2L_{\max}(L_{\max} +\sigma) \tfrac{\sqrt{k} + \gamma }{\sqrt{b}} \nonumber \\
        &\quad \quad \quad \quad + \alpha^4 L_{\max}^3(L_{\max}+\sigma)\tfrac{1 + \gamma}{\sqrt{b}} ) \nonumber \\
        &\quad\vdots  \nonumber \\
        &\leq \|\del_{t}\| + O(\alpha^4 \tau^2 L_{\max}^4 + \alpha^2\tau L_{\max}(L_{\max} +\sigma) \tfrac{\sqrt{k} + \gamma }{\sqrt{b}} \nonumber \\
        &\quad \quad \quad \quad + \alpha^4 \tau L_{\max}^3(L_{\max}+\sigma)\tfrac{1 + \gamma}{\sqrt{b}} ) \nonumber \\
        &= \|\del_{t}\| + O(\alpha^4 \tau^2 L_{\max}^4 + \alpha^2\tau L_{\max}(L_{\max} +\sigma) \tfrac{\sqrt{k} + \gamma }{\sqrt{b}} )...
    \end{align}
\end{proof}

% \begin{lemma}
% Local product does not blow up.
% \end{lemma}

% \begin{proof}
% Recall the notation $\mathbf{e}_{t,i,s}\coloneqq \mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s}- \mathbf{B}_{\ast}\mathbf{w}_{\ast,i}$.

% We have
% \begin{align}
%     \mathbf{e}_{t,i,s+1} &= \mathbf{{B}}_{t,i,s}\mathbf{{w}}_{t,i,s} - \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i} - \alpha\langle \mathbf{w}_{t,i,s}, \mathbf{{w}}_{t,i,s}\rangle\mathbf{\Sigma}_{t,i,s}\mathbf{{e}}_{t,i,s} \nonumber \\
%     &\quad - \alpha \mathbf{{B}}_{t,i,s} \mathbf{B}_{t,i,s}^\top\mathbf{\Sigma}_{t,i,s}\mathbf{{e}}_{t,i,s}  + \alpha^2 \langle \mathbf{w}_{t,i,s}, \mathbf{B}_{t,i,s}^\top\mathbf{\Sigma}_{t,i,s} \mathbf{e}_{t,i,s}\rangle \mathbf{\Sigma}_{t,i,s}\mathbf{{e}}_{t,i,s}  \nonumber \\
%     &= (\mathbf{I}_d -  \alpha \mathbf{{B}}_{t,i,s} \mathbf{B}_{t,i,s}^\top\mathbf{\Sigma}_{t,i,s}  + \alpha^2 \langle \mathbf{w}_{t,i,s}, \mathbf{B}_{t,i,s}^\top\mathbf{\Sigma}_{t,i,s}\mathbf{e}_{t,i,s}\rangle \mathbf{\Sigma}_{t,i,s} - \alpha \| \mathbf{{w}}_{t,i,s}\|_2^2 \mathbf{\Sigma}_{t,i,s} )\mathbf{{e}}_{t,i,s} 
% \end{align}
% thus we need $ \alpha \| \mathbf{{w}}_{t,i,s}\|_2^2 \mathbf{\Sigma}_{t,i,s}\mathbf{{e}}_{t,i,s}  = O(\| \mathbf{{e}}_{t,i,s}\|)$, i.e. $\alpha^2 \|\mathbf{\Sigma}_{t,i,s}\|_2 = O(1)$ (since $\|\mathbf{w}_{t,i,s}\|_2 = \Theta(\sqrt{\alpha})$). But $\|\mathbf{\Sigma}_{t,i,s}\|_2 = O(1+ {d}/{b_i})$. So we need $\alpha = \mathcal{O}(1/\sqrt{d})$.

% Small-sample probabilities:

% $\|\mathbf{\Sigma}_i - \mathbf{I}_k\|_2 \leq d/b$ - easy proof use epsilon-net again.

% \end{proof}



\begin{lemma}[$A_{3,t,i}(s+1)$] \label{lem:la3s}
Distance can get worse locally only by a constant factor.
% For any $t,i,s$,  
\begin{align}
    \dist(\mathbf{B}_{t,i,s}, \mathbf{B}_\ast) &\leq 2  \dist(\mathbf{B}_{t}, \mathbf{B}_\ast)
\end{align}
\end{lemma}

\begin{proof}
Note that
\begin{align}
   \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t,i,s+1}\|_2 &=  \|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_{t,i,s} (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top) \|_2\nonumber \\
   &\leq \|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_{t,i,s} \|_2 \nonumber  \\
   &\quad \vdots \nonumber \\
   &\leq \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t} \|_2
\end{align}
where the first inequality follows since $\|\mathbf{w}_{t,i,s}\|\leq c \sqrt{\alpha}L_{\max}$ (by $A_{1,t,i}(s)$ and $A_{2,t,i}(s)$) and $\alpha$ is sufficiently small, and the last inequality follows by recursively applying the first inequality for all local iterations leading up to $s$.
Thus
\begin{align}
    \dist_{t,i,s} \leq \frac{\|\mathbf{B}_{t}\|_2 }{\sigma_{\min}(\mathbf{B}_{t,i,s})} \dist_{t} \leq \sqrt{\tfrac{1+ \alpha^2 \tau c_{\del}}{1 -  \alpha^2 \tau c_{\del}}} \dist_{t}  \leq 2 \dist_t
\end{align}
where $c_{\del}\coloneqq L_{\max}^2 \kappa_{\max}^2$.
\end{proof}

\subsection{Global induction lemmas}

\begin{lemma}[$A_1(t+1)$] \label{lem:a1fs}

\begin{align}
 \| \mathbf{w}_{t+1} -  \alpha (\mathbf{I}_k& +\del_{t+1})\mathbf{B}_{t+1}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} \|_2 \nonumber \\
 &\leq  c\alpha^{0.5} (L_{\max}+ \sigma) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}}  +  c \alpha^{2.5}\tau L_{\max}^3\nonumber \\
 &\quad +  c\alpha^{2.5}\tau c_{\del}(L_{\max} + \sigma ) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{{Mb}}} + c \alpha^{4.5}\tau^2 L_{\max} c_{\del}^2
\end{align}
\end{lemma}

\begin{proof} We argue similarly to Lemma \ref{lem:a1}. 
Expanding $\mathbf{w}_{t+1}$ yields
\begin{align}
    \mathbf{w}_{t+1} &= \frac{1}{M}\sum_{i=1}^M \mathbf{w}_{t,i,\tau}  \nonumber \\
    &= \frac{1}{M}\sum_{i=1}^M  \del_{t,i,\tau-1}\mathbf{w}_{t,i,\tau-1}  +\alpha \mathbf{B}_{t,i,\tau-1}^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1}  \nonumber \\
    &\quad \quad \quad \quad  + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-1}^\top \mathbf{z}_{t,i,\tau-1}) \nonumber \\
    &= \alpha \mathbf{B}_{t}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} + \frac{1}{M}\sum_{i=1}^M  \del_{t,i,\tau-1}\mathbf{w}_{t,i,\tau-1}    +\alpha (\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_{t})^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \nonumber \\
    &\quad + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1}   + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-1}^\top \mathbf{z}_{t,i,\tau-1}) \nonumber 
    \end{align}
Next, expanding $\mathbf{w}_{t,i,\tau-1}$, we obtain    
    \begin{align}
 \mathbf{w}_{t+1} &= \alpha \mathbf{B}_{t}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}  + \frac{1}{M}\sum_{i=1}^M   \alpha(\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_{t})^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} + \alpha \del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-2}^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}    \nonumber \\
    &\quad 
    % \quad \quad \quad\quad \quad  \quad\quad \quad  \quad\quad \quad 
    + \alpha \del_{t,i,\tau-1} \del_{t,i,\tau-2} \mathbf{w}_{t,i,\tau-2} + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1}   + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-1}^\top \mathbf{z}_{t,i,\tau-1})   \nonumber \\
    &\quad + \alpha \del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-1}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1}   + \alpha \del_{t,i,\tau-1} \mathbf{B}_{t,i,\tau-1}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-1}^\top \mathbf{z}_{t,i,\tau-1}) \nonumber \\
    &= \alpha \mathbf{B}_{t}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} + \alpha \del_{t} \mathbf{B}_{t}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} \nonumber \\
    &\quad + \frac{1}{M}\sum_{i=1}^M   \alpha(\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_{t})^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} + \alpha^2 ( \del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-2}^\top - \del_{t}\mathbf{B}_{t}^\top )\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}  \nonumber \\
    &\quad   +  \del_{t,i,\tau-1} \del_{t,i,\tau-2} \mathbf{w}_{t,i,\tau-2}  + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1}   + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-1}^\top \mathbf{z}_{t,i,\tau-1})   \nonumber \\
    &\quad + \alpha \del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-1}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1}   + \alpha \del_{t,i,\tau-1} \mathbf{B}_{t,i,\tau-1}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-1}^\top \mathbf{z}_{t,i,\tau-1})   \nonumber \\
    &= \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} + \alpha \del_{t+1} \mathbf{B}_{t+1}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} \nonumber \\
    &\quad + \alpha (\mathbf{B}_t -\mathbf{B}_{t+1})^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} + \alpha (\del_t\mathbf{B}_t -\del_{t+1}\mathbf{B}_{t+1})^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}  \nonumber \\
    &\quad + \frac{1}{M}\sum_{i=1}^M   \alpha(\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_{t})^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} + \alpha^2 ( \del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-2}^\top - \del_{t}\mathbf{B}_{t}^\top )\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}  \nonumber \\
    &\quad  +  \del_{t,i,\tau-1} \del_{t,i,\tau-2} \mathbf{w}_{t,i,\tau-2}  + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1}   + \alpha \mathbf{B}_{t,i,\tau-1}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-1}^\top \mathbf{z}_{t,i,\tau-1})   \nonumber \\
    &\quad + \alpha \del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-2}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-2})\mathbf{e}_{t,i,\tau-2}   + \alpha \del_{t,i,\tau-1} \mathbf{B}_{t,i,\tau-2}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-2}^\top \mathbf{z}_{t,i,\tau-2})  \label{chara11}
\end{align}
Therefore
\begin{align}
   & \|\mathbf{w}_{t+1} -  \alpha (\mathbf{I}_k +\del_{t+1})\mathbf{B}_{t+1}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} \|_2 \nonumber \\
   &\leq \alpha L_{\max} \| (\mathbf{B}_t - \mathbf{B}_{t+1})^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t} \|  +  \alpha  L_{\max} \|(\del_t \mathbf{B}_t - \del_{t+1}\mathbf{B}_{t+1})^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}\| \nonumber \\
    &\quad + \alpha\left\|\frac{1}{M}\sum_{i=1}^M   (\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_{t})^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \right\| + \alpha^2\left\|\frac{1}{M}\sum_{i=1}^M   (\del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-2} - \del_t\mathbf{B}_{t})^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}  \right\| \nonumber \\
    &\quad +\left\|\frac{1}{M}\sum_{i=1}^M  \del_{t,i,\tau-1} \del_{t,i,\tau-2} \mathbf{w}_{t,i,\tau-2}  \right\| + \alpha \left\|\frac{1}{M}\sum_{i=1}^M  \mathbf{B}_{t,i,\tau-1}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1} \right\| \nonumber \\
    &\quad + \alpha \left\|\frac{1}{M}\sum_{i=1}^M  \mathbf{B}_{t,i,\tau-1}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-1}^\top \mathbf{z}_{t,i,\tau-1}) \right\| + \alpha \left\|\frac{1}{M}\sum_{i=1}^M\del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-2}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,\tau-2})\mathbf{e}_{t,i,\tau-2}  \right\| \nonumber \\
    &\quad + \alpha \left\|\frac{1}{M}\sum_{i=1}^M \del_{t,i,\tau-1} \mathbf{B}_{t,i,\tau-2}^\top (\tfrac{1}{b} \mathbf{X}_{t,i,\tau-2}^\top \mathbf{z}_{t,i,\tau-2}) \right\| \nonumber \\
    &\leq \alpha L_{\max} \| (\mathbf{B}_t - \mathbf{B}_{t+1})^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t} \|  +  \alpha  L_{\max} \|(\del_t \mathbf{B}_t - \del_{t+1}\mathbf{B}_{t+1})^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}\|  \nonumber \\
    &\quad + \alpha\left\|\frac{1}{M}\sum_{i=1}^M   (\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_{t})^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}  \right\| + \alpha^2\left\|\frac{1}{M}\sum_{i=1}^M   (\del_{t,i,\tau-1}\mathbf{B}_{t,i,\tau-1} - \del_t\mathbf{B}_{t})^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}  \right\| \nonumber \\
    &\quad +c\alpha^{0.5} \|\del\|^2 L_{\max} + c\alpha^{0.5} (L_{\max}+ \sigma) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}}  + c \alpha^{0.5} \|\del_t\| (L_{\max}+\sigma)\tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{b}}\label{march}
\end{align}
where the last inequality follows with probability at least $1-$ by Lemmas \ref{lem:concen1} and \ref{lem:concen2}. To bound the rest of the norms in the RHS of \eqref{march}, we use
\begin{align}
    &\left\|\frac{1}{M}\sum_{i=1}^M \mathbf{B}_{\ast}^\top( \mathbf{B}_{t,i,\tau-1} - \mathbf{B}_{t})\right\|_2\nonumber \\
    &\leq \sum_{s=1}^{\tau-1} \left\|\frac{1}{M}\sum_{i=1}^M \mathbf{B}_{\ast}^\top( \mathbf{B}_{t,i,s}- \mathbf{B}_{t,i,s-1})\right\|_2 \nonumber \\
    &\leq   \alpha\sum_{s=1}^{\tau-1} \|\mathbf{e}_{t,i,s-1}\mathbf{w}_{t,i,s-1}^\top\|_2 +\alpha \sum_{s=1}^{\tau-1} \left\|\frac{1}{M}\sum_{i=1}^M \mathbf{B}_{\ast}^\top (\mathbf{I}_k - \mathbf{\Sigma}_{t,i,s-1})\mathbf{e}_{t,i,s-1}\mathbf{w}_{t,i,s-1}^\top \right\| \nonumber \\
    &\quad + \alpha \sum_{s=1}^{\tau-1} \left\|\frac{1}{M}\sum_{i=1}^M \mathbf{B}_{\ast}^\top (\tfrac{1}{b}\mathbf{X}_{t,i,s-1}^\top\mathbf{z}_{t,i,s-1})\mathbf{w}_{t,i,s-1}^\top \right\|   \nonumber \\
    &\leq  \alpha^{1.5}\tau L_{\max}^2 +  \alpha^{1.5}\tau L_{\max}(L_{\max} + \sigma ) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{{Mb}}} \label{chara22}
\end{align}
where \eqref{chara22} follows with probability at least $1-$. Using this, we obtain
\begin{align}
     \|\mathbf{B}_\ast^\top(\mathbf{B}_{t+1} - \mathbf{B}_{t})\|_2 &=  \left\|\frac{1}{M}\sum_{i=1}^M\mathbf{B}_\ast^\top(\mathbf{B}_{t,i,\tau} - \mathbf{B}_{t})\right\|_2\nonumber \\
     &\leq  c\alpha^{1.5}\tau L_{\max}^2 +  \alpha^{1.5}\tau L_{\max}(L_{\max} + \sigma ) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{{Mb}}}, \nonumber 
     \end{align}
\begin{align}
 & \left\|\frac{1}{M}\sum_{i=1}^M \mathbf{B}_\ast^\top( \mathbf{B}_{t,i,\tau-2}\del_{t,i,\tau-1} - \mathbf{B}_{t}\del_{t})\right\|_2\nonumber \\
 &\leq \left\|\frac{1}{M}\sum_{i=1}^M \mathbf{B}_\ast^\top(\mathbf{B}_{t,i,\tau-2} - \mathbf{B}_{t})\right\|_2 + \alpha\left\|\frac{1}{M}\sum_{i=1}^M\mathbf{B}_\ast^\top(\mathbf{B}_{t,i,\tau-2}\mathbf{B}_{t,i,\tau-1}^\top\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_{t}\mathbf{B}_{t}^\top\mathbf{B}_{t})\right\|_2  \nonumber \\
  &\leq \left\|\frac{1}{M}\sum_{i=1}^M \mathbf{B}_\ast^\top(\mathbf{B}_{t,i,\tau-2} - \mathbf{B}_{t})\right\|_2 +  \alpha\left\|\frac{1}{M}\sum_{i=1}^M\mathbf{B}_\ast^\top(\mathbf{B}_{t,i,\tau-2} - \mathbf{B}_{t})\mathbf{B}_{t,i,\tau-1}^\top\mathbf{B}_{t,i,\tau-1}\right\|_2 \nonumber \\
  &\quad + \alpha \left\| \frac{1}{M}\sum_{i=1}^M\mathbf{B}_t (\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_t)^\top \mathbf{B}_{t,i,\tau-1} \right\|_2  + \alpha \left\| \frac{1}{M}\sum_{i=1}^M\mathbf{B}_t \mathbf{B}_{t}^\top (\mathbf{B}_{t,i,\tau-1} - \mathbf{B}_t)  \right\|_2 \nonumber \\
  &\leq c \alpha^{1.5}\tau L_{\max}^2 +  \alpha^{1.5}\tau L_{\max}(L_{\max} + \sigma ) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{{Mb}}}, \nonumber 
 \end{align}
and, similarly (using $\mathbf{B}_{t+1}= \tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_{t,i,\tau}$),
 \begin{align}
 \|\mathbf{B}_t\del_t - \mathbf{B}_{t+1}\del_{t+1}\|_2 &\leq \left\|\frac{1}{M}\sum_{i=1}^M\mathbf{B}_{t,i,\tau} - \mathbf{B}_{t}\right\|_2 +  \alpha\left\|\frac{1}{M}\sum_{i=1}^M(\mathbf{B}_{t,i,\tau} - \mathbf{B}_{t})\mathbf{B}_{t+1}^\top\mathbf{B}_{t}\right\|_2 \nonumber \\
  &\quad + \alpha \left\| \frac{1}{M}\sum_{i=1}^M\mathbf{B}_t (\mathbf{B}_{t,i,\tau} - \mathbf{B}_t)^\top \mathbf{B}_{t+1} \right\|_2  + \alpha \left\| \frac{1}{M}\sum_{i=1}^M\mathbf{B}_t \mathbf{B}_{t}^\top (\mathbf{B}_{t,i,\tau} - \mathbf{B}_t)  \right\|_2 \nonumber \\
  &\leq c \alpha^{1.5}\tau L_{\max}^2 +  \alpha^{1.5}\tau L_{\max}(L_{\max} + \sigma ) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{{Mb}}}.
\end{align} with probability at least .
Also, we have 
\begin{align}
    \| \del_{t,i,\tau-1} \del_{t,i,\tau-2} \mathbf{w}_{t,i,\tau-2} \|_2 &\leq c \alpha^{4.5} \tau^2 L_{\max} c_{\del}^2
\end{align}
Thus, using \eqref{chara}, we have 
\begin{align}
 \| \mathbf{w}_{t+1} -  \alpha (\mathbf{I}_k& +\del_{t+1})\mathbf{B}_{t+1}^\top \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} \|_2 \nonumber \\
 &\leq  c\alpha^{0.5} (L_{\max}+ \sigma) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}}  +  c \alpha^{2.5}\tau L_{\max}^3\nonumber \\
 &\quad +  c\alpha^{2.5}\tau c_{\del}(L_{\max} + \sigma ) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{{Mb}}} + c \alpha^{4.5}\tau^2 L_{\max} c_{\del}^2
\end{align}
where $c_{\del}\coloneqq L_{\max}^2 \kappa_{\max}^2$ (i.e. $c\alpha^2\tau L_{\max}^2 \kappa_{\max}^2$ upper bounds $\|\del_t\|_2$).
\end{proof}

\input{App_Finite_A2}

\begin{lemma}[$A_3(t+1)$] \label{lem:1a3}
Suppose ... hold, then

\begin{align}
    \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|_2 &\leq (1 - E_0 ... \alpha^2 \tau)\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t}\|_2 + ...
\end{align}
\end{lemma}


\begin{proof}
Let $\mathbf{\tilde{B}}_{t+1}$ denote the update in the population case, namely
\begin{align}
    \mathbf{\tilde{B}}_{t+1} =  \mathbf{{B}}_{t} \left(\frac{1}{n} \sum_{i=1}^n  \prod_{s=0}^{\tau-1}(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top)\right) + \mathbf{{B}}_\ast  \left(\frac{\alpha}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i}  \sum_{s=0}^{\tau-1}\mathbf{w}_{t,i,s}^\top \prod_{r=s+1}^{\tau-1}(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,r}\mathbf{w}_{t,i,r}^\top) \right)
\end{align}
We have 
\begin{align}
    \mathbf{B}_{t+1} &= \tfrac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i,\tau} \nonumber \\
    &= \tfrac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i,\tau-1}\boldsymbol{\delta}_{t,i,\tau-1} + \alpha \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,\tau-1}^\top  +  (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1} \mathbf{w}_{t,i,\tau-1}^\top\nonumber \\
    &= \tfrac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i,\tau-2}\boldsymbol{\delta}_{t,i,\tau-2}\boldsymbol{\delta}_{t,i,\tau-1} + \alpha \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i,\tau-2}^\top \boldsymbol{\delta}_{t,i,\tau-1} + \alpha \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,\tau-1}^\top \nonumber \\
    &\quad + \alpha (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,\tau-2})\mathbf{e}_{t,i,\tau-2} \mathbf{w}_{t,i,\tau-2}^\top \boldsymbol{\delta}_{t,i,\tau-1} + {\alpha} (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,\tau-1})\mathbf{e}_{t,i,\tau-1} \mathbf{w}_{t,i,\tau-1}^\top\nonumber \\
    &= \mathbf{{B}}_{t} \left(\frac{1}{n} \sum_{i=1}^n  \prod_{s=0}^{\tau-1}\boldsymbol{\delta}_{t,i,s}\right) + \mathbf{{B}}_\ast  \left(\frac{\alpha}{n} \sum_{i=1}^n \mathbf{w}_{\ast,i}  \sum_{s=0}^{\tau-1}\mathbf{w}_{t,i,s}^\top \prod_{r=s+1}^{\tau-1}\boldsymbol{\delta}_{t,i,r} \right) \nonumber \\
    &\quad + \frac{\alpha}{n}  \sum_{i=1}^n \sum_{s=1}^\tau  (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})\mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}^\top \prod_{r=s}^\tau \boldsymbol{\delta}_{t,i,r}  \nonumber \\
    &=   \mathbf{\tilde{B}}_{t+1} + \frac{\alpha}{n}  \sum_{i=1}^n \sum_{s=1}^\tau  (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})\mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}^\top \prod_{r=s}^\tau \boldsymbol{\delta}_{t,i,r} 
\end{align}
therefore
\begin{align}
    \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|_2 &\leq \|\mathbf{B}_{\ast,\perp}^\top \mathbf{\tilde{B}}_{t+1}\|_2  + \alpha\left\| \frac{1}{n} \sum_{i=1}^n  \mathbf{B}_{\ast,\perp}^\top \sum_{s=1}^\tau  (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})\mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}^\top \prod_{r=s}^\tau \boldsymbol{\delta}_{t,i,r} \right\|_2
\end{align}
The error term due to the noise can be controlled as
\begin{align}
  \alpha\left\| \frac{1}{n} \sum_{i=1}^n  \mathbf{B}_{\ast,\perp}^\top \sum_{s=1}^\tau  (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})\mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}^\top \prod_{r=s}^\tau \boldsymbol{\delta}_{t,i,r} \right\|_2 
%   &\leq \tau \alpha^{1.5} \tfrac{\sqrt{d}}{\sqrt{nm}} \nonumber \\
  &\leq \alpha\left\| \frac{1}{n} \sum_{i=1}^n   \sum_{s=1}^\tau  (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})\mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}^\top \prod_{r=s}^\tau \boldsymbol{\delta}_{t,i,r} \right\|_2  \nonumber
  \end{align}
  By standard sub-gaussian concentration results, we have that as long as $N= \Omega(d)$. with probability at least $1 - \exp(cd)$.
  \begin{align}
       \alpha  \left\| \frac{1}{n} \sum_{i=1}^n  \sum_{s=1}^\tau (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})\mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}^\top \prod_{r=s}^\tau \boldsymbol{\delta}_{t,i,r} \right\|_2   &\leq c' \alpha \tau \frac{\sqrt{d}}{\sqrt{N}}  \max_{i\in [n], s\in [\tau]} \|\mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top\|_2 \leq c'' \alpha^{1.5}\tau \frac{\sqrt{d}}{\sqrt{N}} L_{\max}^2 \nonumber 
  \end{align}
 for absolute constants $c,c',c''$. %(in fresh samples case)
 
 
 
 
 
Next, we have
\begin{align}
    \|\mathbf{B}_{\ast,\perp}^\top \mathbf{\tilde{B}}_{t+1}\|_2 &=  \left\|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_t \tfrac{1}{M} \sum_{i=1}^M \prod_{s=0}^\tau (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top)\right\|_2  \nonumber \\
    &\leq  \left\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_t \right\|_2 \left\|\mathbf{I}_k -\alpha \mathbf{w}_t\mathbf{w}_t^\top\right\| \left\| \tfrac{1}{M} \sum_{i=1}^M \prod_{s=1}^\tau (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top)\right\|_2      \nonumber
    % (1 - 0.4\alpha^2 E_0 \mu_\ast^2 \tau)\|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t}\|_2.
\end{align}
 
 We can expand the right product of $\mathbf{B}_t (\mathbf{I} - \alpha \mathbf{w}_t \mathbf{w}_t^\top)$ using the binomial expansion as follows:
\begin{align}
\frac{1}{n} \sum_{i=1}^n  \prod_{s=1}^{\tau-1}(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top) &=  \mathbf{I}_k - \frac{\alpha}{n} \sum_{i=1}^n  \sum_{s = 1}^{\tau-1} \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top + \frac{\alpha^2}{n} \sum_{i=1}^n \sum_{s=1}^{\tau-2} \sum_{s^{(1)}=s+1}^{\tau-1}  \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top\mathbf{w}_{t,i,s^{(1)}}\mathbf{w}_{t,i,s^{(1)}}^\top \nonumber \\
&\quad - \dots + \sign(\tau)\frac{\alpha^{\tau}}{n} \sum_{i=1}^n \prod_{s=1}^{\tau-1}  \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top  \nonumber
\end{align}
Recall that each $\|\mathbf{w}_{t,i,s}\|_2 = \mathcal{O}(\sqrt{\alpha}L_{\max})$. Thus, after the identity, the spectral norm of the first set of summations scales as $\mathcal{O}(\alpha^2 \tau L_{\max}^2 )$, the second set scales as $\mathcal{O}(\alpha^4 \tau^2 L_{\max}^4)$, and so on. 
We in fact use the first set of summations as a negative term, and bound all subsequent sets of summations as errors, exploiting the fact that their norms are geometrically decaying. In particular, we have:
\begin{align}
    \left\|\frac{1}{n} \sum_{i=1}^n  \prod_{s=1}^{\tau-1}(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top)  \right\|_2 &\leq \left\| \mathbf{I}_k - \frac{\alpha}{n} \sum_{i=1}^n   \sum_{s = 1}^{\tau-1} \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top \right\|_2 + \sum_{z=2}^{\tau-1}(\alpha^2 \tau L_{\max}^2)^z \nonumber \\ %+ \dots \nonumber \\
    &\leq  \left\| \mathbf{I}_k - \frac{\alpha}{n} \sum_{i=1}^n   \sum_{s = 1}^{\tau-1} \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top \right\|_2 +  \frac{\alpha^4 \tau^2 L_{\max}^4}{1 - \alpha^2 \tau L_{\max}^2} \label{sslast}
    \end{align}
Next, we use $\mathbf{w}_{t,i,s} = \alpha \mathbf{B}_{t,i,s-1}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} + \del_{t,i,s-1}\mathbf{w}_{t,i,s-1}$ for all $s\geq 1$, where $\|\del_{t,i,s-1}\mathbf{w}_{t,i,s-1}\|_2 \leq c\sqrt{\alpha} \|\del_{t}\|_2 L_{\max}\leq c \alpha^{2.5} \tau L_{\max} c_{\del}$ to obtain 
\begin{align}
   \left\| \mathbf{I}_k - \frac{\alpha}{n} \sum_{i=1}^n   \sum_{s = 1}^{\tau-1} \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top \right\|_2 &\leq  \left\| \mathbf{I}_k - \frac{\alpha^3}{n} \sum_{i=1}^n   \sum_{s = 1}^{\tau-1} \mathbf{B}_{t,i,s-1}^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top\mathbf{B}_{t,i,s-1} \right\|_2 \nonumber \\
   &\quad + \alpha^2\tau^2 L_{\max}^2 \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{N}}  + 3 c \alpha^4 \tau^2 L_{\max}^2 c_{\del}\label{slast}
   \end{align}
 Next, we have for any $s-1 \in \{1,\dots,\tau-1\}$, 
 \begin{align}
    \| \mathbf{B}_{t,i,s-1} - \mathbf{B}_t \|_2 = \| \mathbf{B}_{t,i,s-1} - \mathbf{B}_{t,i,0} \|_2  &\leq \sum_{r = 1}^{s-1} \| \mathbf{B}_{t,i,r} - \mathbf{B}_{t,i,r-1} \|_2 \nonumber \\
    &\leq \alpha \sum_{r = 1}^{s-1} \|\mathbf{e}_{t,i,r-1}\|_2 \|\mathbf{w}_{t,i,r-1}\|_2 \nonumber \\
    &\leq c'\alpha^{1.5} (\tau-1) L_{\max}^2 \nonumber
 \end{align}
 Thus we have 
   \begin{align}
 \bigg\| \mathbf{I}_k - \frac{\alpha^3}{n} \sum_{i=1}^n   &\sum_{s = 1}^{\tau-1} \mathbf{B}_{t,i,s-1}^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top\mathbf{B}_{t,i,s-1} \bigg\|_2  \nonumber \\
 &\leq  \left\| \mathbf{I}_k - \frac{\alpha^3}{n} \sum_{i=1}^n   \sum_{s = 1}^{\tau-1} \mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top\mathbf{B}_{t} \right\|_2 \nonumber \\
 &\quad  + \left\|\frac{\alpha^3}{n} \sum_{i=1}^n   \sum_{s = 1}^{\tau-1} (\mathbf{B}_{t} - \mathbf{B}_{t,i,s-1} )^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top\mathbf{B}_{t,i,s-1} \right\|_2  \nonumber \\
 &\quad + \left\|\frac{\alpha^3}{n} \sum_{i=1}^n   \sum_{s = 1}^{\tau-1} \mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top(\mathbf{B}_t - \mathbf{B}_{t,i,s-1}) \right\|_2  \nonumber\\
 &\leq  \left\| \mathbf{I}_k - \frac{\alpha^3}{n} \sum_{i=1}^n   \sum_{s = 1}^{\tau-1} \mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top\mathbf{B}_{t} \right\|_2 + 2c \alpha^4 \tau^2  L_{\max}^4 \nonumber \\
 &\leq 1 - \alpha^2 (\tau-1) E_0 \mu_\ast^2 + 2c \alpha^4 (\tau -1)^2  L_{\max}^4  \label{last}
    % &\quad + 2 \tau^2 \alpha^4 L_{\max}^4  \nonumber \\ %+ 3 \tau \alpha^2 L_\ast^2 \max_{i,s}\|\del_{t,i,s}\|_2 \nonumber \\
    % &\leq  1 - (1-\tilde{c})\tau \alpha^2 \mu_\ast^2 E_0 + 2 \tau^2 \alpha^4 L_{\max}^4 + 3 \tau \alpha^2 L_\ast^2 \max_{i,s}\|\del_{t,i,s}\|_2 \nonumber
\end{align}
 
 


%  for non-fresh samples, but not worrying about independence issues, we will get just $\sqrt{d/N}$ + uniform error
 
%  also, local errors will be $\sqrt{k}/\sqrt{n}$ + uniform

%  {\color{red} we can do better in terms of $\tau$ in the FS case. no we cant because that requires taking the max of the subgaussian norms. we need tighter in terms of norms.}
%  We can further bound $c'' \alpha^{1.5} \tau \frac{\sqrt{d}}{\sqrt{N}} L_{\max}^2 \leq bstar perp bt$....  write as proportional to dist

% We can't say that $\|\mathbf{e}_{t,i,s}\|_2$ is a function of $\dist_{t,i,s}$ because $\dist_{t,i,s}$ may blow up if not projected onto something smaller.
% \begin{align}
    
% \end{align}

% {\color{red} we have $n$ isotropic gaussian independent random vectors in $\mathbb{R}^k$. How large do $n$ and $b$ need to be to ensure that a subset of $b$ vectors chosen uniformly is satisfies that its gram matrix is close to the gram matrix of the $n$ vectors with high probability?

% fine.


% it seems like having non-fresh samples at each iteration is not an issue but i am not convinced....





% we need invoke k-dim concentration result $\tau T = \tau \log(1/\epsilon)$ times, which is fine. will get a $\log(\tau)$
% }



\end{proof}



\begin{lemma}[$A_4(t+1)$] \label{lem:la4}
Distance is converging at rate
\end{lemma}

\begin{proof}

fresh samples every time:
\begin{align}
    \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t+1}\|_2 &\leq ( 1 - \alpha^2 \tau) \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t}\|_2  + \alpha^{1.5} \frac{\sqrt{d\tau}}{\sqrt{N}} \nonumber \\
    &\leq (1 - \alpha^2 \tau)^{t} \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{0}\|_2 + \alpha^{1.5} \frac{\sqrt{d\tau}}{\sqrt{N}} \sum_{s = 1}^t (1 - \alpha^2 \tau)^s
\end{align}

\begin{align}
    \dist_{t+1} &\leq c (1 - \alpha^2 \tau) \dist_0 + \frac{\alpha^2 \sqrt{d \tau}}{(1-\|\del\|_2)\alpha^2 \tau \sqrt{N}} \leq c (1 - \alpha^2 \tau) \dist_0 + \frac{ \sqrt{d}}{(1-\|\del\|_2) \sqrt{N\tau}}
\end{align}

\begin{align}
    
    
\end{align}
\end{proof}





\begin{lemma}

\end{lemma}

\begin{proof}

\end{proof}


-------


\begin{align}\nabla_{\mathbf{B}} \hat{f}_{t,i,s}(\mathbf{B}_{t,i,s}, \mathbf{w}_{t,i,s}; \mathbf{X}_{t,i,s}) &=  \mathbf{{\Sigma}}_{t,i,s} (\mathbf{B}_{t,i,s} \mathbf{w}_{t,i,s} - \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i}) \mathbf{w}_{t,i,s}^\top \nonumber \\
&= (\mathbf{B}_{t,i,s} \mathbf{w}_{t,i,s} 
-  \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i}) \mathbf{w}_{t,i,s}^\top  - (\mathbf{I}_d-\mathbf{{\Sigma}}_{t,i,s})( \mathbf{B}_{t,i,s} \mathbf{w}_{t,i,s} 
-  \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i}  )\mathbf{w}_{t,i,s}^\top \nonumber \\
\nabla_{\mathbf{w}}\hat{f}_{t,i,s}(\mathbf{B}_{t,i,s}, \mathbf{w}_{t,i,s}; \mathbf{X}_{t,i,s}) &=  \mathbf{B}_{t,i,s}^\top\mathbf{{\Sigma}}_{t,i,s} (\mathbf{B}_{t,i,s} \mathbf{w}_{t,i,s} - \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i}) \nonumber \\
&= \mathbf{B}_{t,i,s}^\top (\mathbf{B}_{t,i,s} \mathbf{w}_{t,i,s} 
-  \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i})- \mathbf{B}_{t,i,s}^\top (\mathbf{I}_d-\mathbf{{\Sigma}}_{t,i,s})( \mathbf{B}_{t,i,s} \mathbf{w}_{t,i,s} 
-  \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i}  )\nonumber \\
\mathbf{e}_{t,i,s}
\end{align}

\begin{align}
    \mathbf{B}_{t+1} &= \tfrac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i,\tau-1}(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,\tau-1}\mathbf{w}_{t,i,\tau-1}^\top) + \alpha \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,\tau-1}^\top \nonumber \\
    &\quad + \tfrac{1}{n}\sum_{i=1}^n (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,\tau-1})(\mathbf{B}_{t,i,\tau-1}\mathbf{w}_{t,i,\tau-1} - \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}) \mathbf{w}_{t,i,\tau-1}^\top\nonumber \\
    &= \tfrac{1}{n}\sum_{i=1}^n \mathbf{B}_{t,i,\tau-2}(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,\tau-2}\mathbf{w}_{t,i,\tau-2}^\top)(\mathbf{I}_k - \alpha \mathbf{w}_{t,i,\tau-1}\mathbf{w}_{t,i,\tau-1}^\top) \nonumber \\
    &\quad + \alpha \mathbf{B}_{\ast} \mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i,\tau-2}^\top (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,\tau-1}\mathbf{w}_{t,i,\tau-1}^\top) + \alpha \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,\tau-1}^\top \nonumber \\
    &\quad + \tfrac{\alpha}{n}\sum_{i=1}^n (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,\tau-2})(\mathbf{B}_{t,i,\tau-2}\mathbf{w}_{t,i,\tau-2} - \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}) \mathbf{w}_{t,i,\tau-2}^\top (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,\tau-1}\mathbf{w}_{t,i,\tau-1}^\top)\nonumber\\
    &\quad + \tfrac{\alpha}{n}\sum_{i=1}^n (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,\tau-1})(\mathbf{B}_{t,i,\tau-1}\mathbf{w}_{t,i,\tau-1} - \mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}) \mathbf{w}_{t,i,\tau-1}^\top\nonumber
\end{align}
Error terms will accumulate as:
\begin{align}
  \left\|   \sum_{s=1}^\tau \tfrac{\alpha}{n} \sum_{i=1}^n (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})\mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}^\top \prod_{r=s}^\tau (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,r}\mathbf{w}_{t,i,r}^\top) \right\|_2 &\leq \tau \alpha^{1.5} \tfrac{\sqrt{d}}{\sqrt{nm}}
\end{align}
which is fine.

Local updates:
\begin{align}
\mathbf{B}_{t,i,s+1} &= \mathbf{B}_{t,i,s} - \alpha \mathbf{\hat{G}}_{t,i,s} \nonumber \\ 
\mathbf{\hat{G}}_{t,i,s} &= (\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top - (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top \nonumber \\
    \del_{t,i,s+1} &= \del_{t,i,s} + \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{\hat{G}}_{t,i,s} + \alpha^2 \mathbf{\hat{G}}_{t,i,s}^\top \mathbf{B}_{t,i,s} - \alpha^3  \mathbf{\hat{G}}_{t,i,s}^\top \mathbf{\hat{G}}_{t,i,s}  \nonumber \\
    &= \del_{t,i,s} + \alpha^2 \mathbf{B}_{t,i,s}^\top (\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top + \alpha^2 \mathbf{w}_{t,i,s}(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})^\top \mathbf{B}_{t,i,s} \nonumber \\
    &\quad - \alpha^3 \|\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\|_2^2 \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top  \nonumber \\
    &\quad - \alpha^2 \mathbf{B}_{t,i,s}^\top (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top \nonumber \\
    &\quad - \alpha^2 \mathbf{w}_{t,i,s}\left((\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\right)^\top \mathbf{B}_{t,i,s} \nonumber \\
    &\quad + \alpha^2\mathbf{w}_{t,i,s}\left((\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\right)^\top\left((\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s})(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\right) \mathbf{w}_{t,i,s}^\top \nonumber \\
    % &\quad + \alpha^2 cross terms \nonumber  \\
   \| \del_{t,i,s+1}\|_2 &\leq  \| \del_{t,i,s}\|_2 + \alpha^4 \|\mathbf{e}_{t,i,s}\|_2^2 L_{\max}^2 + \alpha^2 \tfrac{\sqrt{k}+\sqrt{\log(n)}}{\sqrt{m}}\|\mathbf{e}_{t,i,s}\|_2 \nonumber \\
   \|\mathbf{e}_{t,i,s+1}\|_2 &\leq (1 - \alpha^2 \|\mathbf{\Sigma}_{t,i,s}\|_2 \|\mathbf{w}_{\ast,t,i}\|_2^2)\|\mathbf{e}_{t,i,s}\|_2 \nonumber \\
   \mathbf{w}_{t,i,s+1} &= \del_{t,i,s}\mathbf{w}_{t,i,s}  +\alpha \mathbf{B}_{t,i,s}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i} + 
\end{align}
Need $\alpha^2 (1+ \tfrac{\sqrt{d}}{\sqrt{m}})\|\mathbf{w}_{\ast,t,i}\|_2^2$

% bottleneck: cannot have local convergence with less than d samples per task.
% check empirically if it works

% we need these things:

% wtis is close to alpha Btis Bstar wstar
% - easy because everything is dimension k

% wtis = goodi + badi
%  badi badi is going to be a problem. its fine use technique from maml anil paper.
%  but does first order approx really dominate
%  now we need to deal with higher order moments 
 
%  (1/n sum badi badi) (1/n sum badi' badi')
%  = bad-i bad-i
 
% 1/n sum-i=1n (1 - xi1 xi1)(1 - xi2 xi2)(1 - xi3 xi3)
 
% 1/n sum-i=1n sum-s=13 xis xis --> tau alpha2 

% 1/n sum-i=1n sum-s=13 xis xis sum-s'=13 xis' xis'

% Btis is well-conditioned





Need $\alpha = O(1/\sqrt{d})$. There is no getting around this. 

But we can choose $\tau = d$. But then we need to invoke concentration lemma d times. This is fine because it fails with exp small probability. Succeeds with prob $1 - e^{-n_i}$. Now, $1 - de^{-n_i}$ --> need $n_i = \Theta(\log(d))$. How many times do we need to invoke in total?

$ (1 - alpha2 \tau)^T \leq \epsilon$ --> $\poly(\kappa)\log(1/\epsilon)$ iters. Thus we need to invoke $$d\poly(\kappa)\log(1/\epsilon)$$ times.


\subsection{Proof of Proposition \ref{cor:1}}

\begin{proof}
Let $\mathbf{e}_{M+1,s} := \mathbf{B}_{T,M+1,s}\mathbf{w}_{T,M+1,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,M+1}$ be the error for Client $M+1$ after fine-tuning the model trained by FedAvg for $T$ rounds. 
For any $s$, note that $\mathbf{e}_{T,M+1,s}\coloneqq \mathbf{B}_{T,M+1,s}\mathbf{w}_{T,M+1,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,M+1}$ can be written as:
\begin{align}
\mathbf{e}_{T,M+1,s+1} = \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top \mathbf{e}_{T,M+1,s+1} + (\mathbf{I}_k - \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top) \mathbf{e}_{T,M+1,s+1} 
\end{align}
where
\begin{align}
 (\mathbf{I}_k - \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top) \mathbf{e}_{T,M+1,s} &=  (\mathbf{I}_k - \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top) \mathbf{B}_{\ast} \mathbf{w}_{\ast,M+1} \leq \dist_T \|\mathbf{w}_{\ast,M+1}\|_2. 
\end{align}
by the Cauchy-Schwarz Inequality and the fact that $\|(\mathbf{I}_k - \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top) \mathbf{B}_{\ast}\|_2 = \dist_T$. On the other hand,
% We consider the evolution of the projection of $\mathbf{e}_{M+1,s}$ onto the column space of $\mathbf{B}_T$.

% $\mathbf{z}_{T,M+1,s}\in \mathbb{R}^{b}$

% $ \alpha \mathbf{B}_{t,i,s}^\top \mathbf{X}_{t,i,s}^\top\mathbf{z}_{T,M+1,s}$

% $ \alpha \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}\mathbf{w}_{T,M+1,s}^\top$
\begin{align}
    &\mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top \mathbf{e}_{M+1,s+1} \nonumber \\
    &=  \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top \big(\mathbf{I}_d -  \alpha \mathbf{{B}}_{T,M+1,s} \mathbf{B}_{T,M+1,s}^\top\mathbf{\Sigma}_{T,M+1,s}  + \alpha^2 \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{\Sigma}_{T,M+1,s}\mathbf{e}_{T,M+1,s}\rangle \mathbf{\Sigma}_{T,M+1,s} \nonumber \\
    &\quad  - \alpha \| \mathbf{{w}}_{T,M+1,s}\|_2^2 \mathbf{\Sigma}_{T,M+1,s} \big) \mathbf{e}_{T,M+1,s}  
    - \alpha  \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top\mathbf{B}_{t,M+1,s+1}\mathbf{B}_{T,M+1,s}^\top \tfrac{1}{b}\mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}\nonumber \\
    &\quad - \alpha \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top \tfrac{1}{b}\mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}\langle\mathbf{w}_{T,M+1,s},\mathbf{w}_{t,i,s+1}\rangle \nonumber \\
    &= \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top \big(\mathbf{I}_d -  \alpha \mathbf{{B}}_{T,M+1,s} \mathbf{B}_{T,M+1,s}^\top + \alpha^2 \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{e}_{T,M+1,s}\rangle \mathbf{I}_d   - \alpha \| \mathbf{{w}}_{T,M+1,s}\|_2^2 \mathbf{I}_{d} \big)\mathbf{e}_{T,M+1,s} \nonumber \\
    &\quad + \alpha \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top\mathbf{{B}}_{T,M+1,s} \mathbf{B}_{T,M+1,s}^\top (\mathbf{\Sigma}_{T,M+1,s}- \mathbf{I}_d)\mathbf{e}_{T,M+1,s} \nonumber \\
    &\quad - \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top( \alpha^2 \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{e}_{T,M+1,s}\rangle \mathbf{I}_{d} \nonumber \\
    &\quad -  \alpha^2 \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{\Sigma}_{T,M+1,s}\mathbf{e}_{T,M+1,s}\rangle \mathbf{\Sigma}_{T,M+1,s} )\mathbf{e}_{T,M+1,s}  \nonumber \\
    &\quad  +  \alpha \| \mathbf{{w}}_{T,M+1,s}\|_2^2 \mathbf{\hat{B}}_{T} \mathbf{\hat{B}}_{T}^\top(\mathbf{I}_d - \mathbf{\Sigma}_{T,M+1,s} ) \mathbf{e}_{T,M+1,s} \nonumber \\
    &\quad - \alpha  \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top\mathbf{B}_{t,M+1,s+1}\mathbf{B}_{T,M+1,s}^\top \tfrac{1}{b}\mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s} - \alpha \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top \tfrac{1}{b}\mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}\langle\mathbf{w}_{T,M+1,s},\mathbf{w}_{t,i,s+1}\rangle
\end{align} The terms in the first two lines of the last equation are equivalent to the update in the population case. Define $\mathbf{P}_{\mathbf{B}_{T,M+1,s}} \coloneqq \mathbf{I}_d - \mathbf{\hat{B}}_{T,M+1,s}\mathbf{\hat{B}}_{T,M+1,s}^\top$
These terms can be bounded as
\begin{align}
&\|\mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top \big(\mathbf{I}_d -  \alpha \mathbf{{B}}_{T,M+1,s} \mathbf{B}_{T,M+1,s}^\top + \alpha^2 \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{e}_{T,M+1,s}\rangle \mathbf{I}_d   - \alpha \| \mathbf{{w}}_{T,M+1,s}\|_2^2 \mathbf{I}_{d} \big)\mathbf{e}_{T,M+1,s}\|_2 \nonumber \\
    &= \|\mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top \big(\mathbf{P}_{\mathbf{B}_{T,M+1,s}} + \mathbf{\hat{B}}_{T,M+1,s} \mathbf{\hat{B}}_{T,M+1,s}^\top - \alpha \mathbf{{B}}_{T,M+1,s} \mathbf{B}_{T,M+1,s}^\top + \alpha^2 \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{e}_{T,M+1,s}\rangle \mathbf{I}_d \nonumber \\
    &\quad  - \alpha \| \mathbf{{w}}_{T,M+1,s}\|_2^2 \mathbf{I}_{d} \big)\mathbf{e}_{T,M+1,s}\|_2 \nonumber \\
    &\leq \|\mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top\mathbf{P}_{\mathbf{B}_{T,M+1,s}} 
    % - \alpha^2 \|\mathbf{w}_{\ast,M+1}\|_2^2) 
    \mathbf{B}_\ast \mathbf{w}_{\ast,i} \|_2 +  ( \|\del_{T,M+1,s}\|_2 + c \alpha^2 L^2  )\|\mathbf{e}_{T,M+1,s}\|_2     \nonumber \\
    % \|''\|&\leq \|\mathbf{B}_T^\top\tilde{\del}_{T,M+1,s}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i} \|_2 +  ( \|\del_{T,M+1,s}\|_2 + c \alpha^2 L^2  )\|\mathbf{e}_{T,M+1,s}\|_2 \nonumber \\
    &\leq \min(1, \alpha^2 \tau' L_l^2 ) L_l \dist_T  +  \|\del\| \|\mathbf{e}_{T,M+1,s}\|_2 
\end{align}
% IF WE TRY FOR 1- \alpha^2, we have to deal with fact that we no longer have dif of vectors in the negative term.. but how did we deal with this in pop case?




% Thus 
% \begin{align}
%     \|\mathbf{B}_{T}^\top \mathbf{e}_{M+1,s+1} \|_2
% \end{align}
% \begin{align}
% \|\mathbf{q}_{t,M+1,s+1}\| \leq  (1 - alpha^2 ||w_{\ast,M+1}||^2 ) 2\dist_T + alpha^2 \tau \|\mathbf{q}_{t,M+1,s+1}\|_2 + 
% \end{align}
% To get this, decompose B* into part on the col space of B and orthogonal part
% Orthogonal gets the 1 - alpha2 but it is only as large as dist
% Parallel part gets killed
% Alternatively, could bound it by $||B_T - B_{T,M+1,s}\| \dist —> min$
% The last two terms in the prod error are fine - will have a $+\alpha^{1.5} L^3 \frac{\sqrt{k}+ \sqrt{\log(M\tau)}}{\sqrt{b}}$ error

% The only difficult part is the $BB^T Sig$

% Write as  $-\mathbf{\hat{B}}_{T,M+1,s} \mathbf{\hat{B}}_{T,M+1,s}^\top(\mathbf{I}_d - \mathbf{\Sigma}_{T,M+1,s})$

% $  +  (\mathbf{\hat{B}}_{T,M+1,s} \mathbf{\hat{B}}_{T,M+1,s}^\top  - \mathbf{B}_{T,M+1,s}\mathbf{B}_{T,M+1,s}^T)(\mathbf{I}_d - \mathbf{\Sigma}_{T,M+1,s})$

% Second part is fine, decompose
% $\mathbf{B}_{T,M+1,s}\mathbf{B}_{T,M+1,s}^T = \mathbf{\hat{B}}_{T,M+1,s}\mathbf{R}_{T,M+1,s}\mathbf{R}_{T,M+1,s}^T \mathbf{\hat{B}}_{T,M+1,s}^\top$

% where $\mathbf{\hat{B}}_{T,M+1,s}\mathbf{R}_{T,M+1,s} = \mathbf{B}_{T,M+1,s}$ is the QR-decomposition of $\mathbf{B}_{T,M+1,s}$. 

% For the first part,


Now we consider the finite-sample error terms. We have
\begin{align}
    \|\alpha \mathbf{\hat{B}}_{T}&\mathbf{\hat{B}}_{T}^\top\mathbf{{B}}_{T,M+1,s} \mathbf{B}_{T,M+1,s}^\top (\mathbf{\Sigma}_{T,M+1,s}- \mathbf{I}_d)\mathbf{e}_{T,M+1,s} \|_2
    \leq c \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{b}} \|\mathbf{e}_{T,M+1,s} \|_2, \nonumber 
\end{align}
and 
\begin{align}
     &\alpha^2 \|\mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top(  \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{e}_{T,M+1,s}\rangle \mathbf{I}_{d} - \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{\Sigma}_{T,M+1,s}\mathbf{e}_{T,M+1,s}\rangle \mathbf{\Sigma}_{T,M+1,s} )\mathbf{e}_{T,M+1,s} \| \nonumber \\
     &\leq   \alpha^2 |\langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{e}_{T,M+1,s}\rangle| \|\mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top(   \mathbf{I}_{d} - \mathbf{\Sigma}_{T,M+1,s})\mathbf{e}_{T,M+1,s} \|_2 \nonumber \\
     &\quad + \alpha^2 |\langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top(\mathbf{I}_k - \mathbf{\Sigma}_{T,M+1,s})\mathbf{e}_{T,M+1,s}\rangle|\|\mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top \mathbf{\Sigma}_{T,M+1,s}\mathbf{e}_{T,M+1,s} \|_2\nonumber \\
     &\leq c\alpha^2 L^2 \tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}} \|\mathbf{e}_{T,M+1,s}\|_2,
    %  \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top\mathbf{\Sigma}_{T,M+1,s}\mathbf{e}_{T,M+1,s}\rangle \mathbf{\Sigma}_{T,M+1,s} )\mathbf{e}_{T,M+1,s} \|
\end{align}
and
\begin{align}
    \alpha \| \mathbf{{w}}_{T,M+1,s}\|_2^2 \|\mathbf{\hat{B}}_{T} \mathbf{\hat{B}}_{T}^\top(\mathbf{I}_d - \mathbf{\Sigma}_{T,M+1,s} ) \mathbf{e}_{T,M+1,s}\|_2 &\leq c\alpha^2 L^2 \tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}} \|\mathbf{e}_{T,M+1,s}\|_2
\end{align}
all with high probability. Further, 
note that the noise terms can be written as
\begin{align}
     &\tfrac{\alpha}{b} \mathbf{B}_{t,i,s+1}\mathbf{B}_{T,M+1,s}^\top \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s} \nonumber \\
     &= \tfrac{\alpha}{b} \mathbf{B}_{T,M+1,s}\mathbf{B}_{T,M+1,s}^\top \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s} - \tfrac{\alpha^2}{b}(\mathbf{w}_{T,M+1,s}^\top \mathbf{B}_{T,M+1,s}^\top \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}) \mathbf{e}_{T,M+1,s}   \nonumber \\
     &\quad  - \tfrac{\alpha^2}{b} (\mathbf{w}_{T,M+1,s}^\top \mathbf{B}_{T,M+1,s}^\top \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s})  (\mathbf{I}_d - \mathbf{\Sigma}_{T,M+1,s})\mathbf{e}_{T,M+1,s}      \nonumber \\
     &\quad + \tfrac{\alpha^2}{b^2} (\mathbf{w}_{T,M+1,s}^\top \mathbf{B}_{T,M+1,s}^\top \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}) \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s} \nonumber 
     \end{align}
     and 
     \begin{align}
   & \tfrac{\alpha}{b} \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}\langle\mathbf{w}_{T,M+1,s},\mathbf{w}_{t,i,s+1}\rangle \nonumber \\
   &=  \tfrac{\alpha}{b} \|\mathbf{w}_{T,M+1,s}\|_2^2 \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s} - \tfrac{\alpha^2}{b} \langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{T,M+1,s}^\top \mathbf{\Sigma}_{T,M+1,s} \mathbf{e}_{T,M+1,s}\rangle \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}  \nonumber \\
     &\quad \quad - \tfrac{\alpha^2}{b^2}\langle \mathbf{w}_{T,M+1,s}, \mathbf{B}_{t,M+1,s}^\top \mathbf{X}_{T,M+1,s}^\top \mathbf{z}_{t,M+T,s}\rangle\mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}  \nonumber 
\end{align}
thus, if $b \geq k+\log$,
\begin{align}
    \| \tfrac{\alpha}{b} \mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top&\mathbf{B}_{t,i,s+1}\mathbf{B}_{T,M+1,s}^\top \mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}\| \nonumber \\
    &\leq c \tfrac{\sigma(\sqrt{k}+\sqrt{\log})}{\sqrt{b}} + c \alpha^2 \tfrac{L\sigma(\sqrt{k}+\sqrt{\log})}{\sqrt{b}} \|\mathbf{e}_{T,M+1,s}\|_2  + c \alpha^2 \tfrac{L\sigma^2({k}+{\log})}{{b}} \nonumber \\
    \|\tfrac{\alpha}{b}\mathbf{\hat{B}}_{T}\mathbf{\hat{B}}_{T}^\top&\mathbf{X}_{T,M+1,s}^\top\mathbf{z}_{T,M+1,s}\langle\mathbf{w}_{T,M+1,s},\mathbf{w}_{t,i,s+1}\rangle \| \nonumber \\
    &\leq c \alpha^2 \tfrac{L^2\sigma(\sqrt{k}+\sqrt{\log})}{\sqrt{b}} + c \alpha^2 \tfrac{(L+\sigma)\sigma({k}+ {\log})}{{b}} \|\mathbf{e}_{T,M+1,s}\|_2.   \nonumber 
\end{align}
with high probability.
Putting these together and using $\alpha^2 (L+\sigma)^2 \leq 1$, we have that all of the stochastic terms can be bounded by
\begin{align}
   c\tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}} (\sigma+ \|\mathbf{e}_{T,M+1,s}\|_2),  \nonumber
\end{align}
Combining all terms in the projection onto the column space of $\mathbf{B}_T$, we obtain
\begin{align}
   \|\mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top \mathbf{e}_{T,M+1,s+1}\| &\leq \min(1, \alpha^2 \tau' L_l^2 ) L_l \dist_T  +  c \alpha^2 L^2 \kappa^2 \|\mathbf{e}_{T,M+1,s}\|_2 +c\tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}} (\sigma+ \|\mathbf{e}_{T,M+1,s}\|_2) \nonumber \\
   &\leq +c\tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}}  \|\mathbf{e}_{T,M+1,s}\|_2 +  \min(1, \alpha^2 \tau' L_l^2 ) L_l \dist_T   + c \sigma \tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}}  \nonumber
\end{align}
for an absolute constant $c$. Recursively applying this inequality yields
\begin{align}
    \|\mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top \mathbf{e}_{T,M+1,s+1}\| &\leq \big(\tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}}  \big)^s \|\mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top \mathbf{e}_{T,M+1,s}\| + \sum_{r = 1}^s \big(\tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}} \big)^{s-r} (\dist_T + \sigma \tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}} ) \nonumber \\
    &\leq \big(\tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}}  \big)^s c L + c\tfrac{\sqrt{b}}{\sqrt{b} - \sqrt{k} - \sqrt{\log()}}(\dist_T + \sigma \tfrac{\sqrt{k}+\sqrt{\log}}{\sqrt{b}} ) \nonumber 
\end{align}


{

Need to show:

\begin{align}
    \|(\mathbf{B}_T-\mathbf{B}_{T,M+1,s})^\top(\mathbf{I}_k -  \mathbf{\hat{B}}_{T,M+1,s} \mathbf{\hat{B}}_{T,M+1,s}^\top)\mathbf{B}_\ast  \| &\leq \alpha^{1.5} s \dist_T
\end{align}

major issue: only projected distance stays small locally. so we do not know for sure if the above expression is proportional to the distance...


... we can get an $\alpha^4 \tau^2$ term for the population terms in the finite-sample case. But this is not good enough. 


\begin{align}
    &\|\mathbf{B}_t^\top (\mathbf{I}_d - \alpha \mathbf{B}_{t,i,s} \mathbf{B}_{t,i,s}^\top)(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\| \nonumber \\
    &\leq \|\mathbf{B}_t^\top (\mathbf{I}_d - \alpha \mathbf{B}_{t} \mathbf{B}_{t}^\top)(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\|  \nonumber \\
    &\quad + \alpha\|\mathbf{B}_t^\top (\mathbf{B}_{t} \mathbf{B}_{t}^\top - \mathbf{B}_{t,i,s} \mathbf{B}_{t,i,s}^\top)(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\|  \nonumber \\
    &\leq \|\mathbf{B}_t^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t} \mathbf{\hat{B}}_{t}^\top + \mathbf{\hat{B}}_{t} \mathbf{\hat{B}}_{t}^\top -\alpha \mathbf{B}_{t} \mathbf{B}_{t}^\top)(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\|  \nonumber \\
    &\quad + \alpha\|\mathbf{B}_t^\top (\mathbf{B}_{t} \mathbf{B}_{t}^\top - \mathbf{B}_{t} \mathbf{B}_{t,i,s}^\top)(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}) \|\nonumber \\
    &\quad + \alpha\| \mathbf{B}_t^\top(\mathbf{B}_{t} \mathbf{B}_{t,i,s}^\top- \mathbf{B}_{t,i,s} \mathbf{B}_{t,i,s}^\top)(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,t,i})\|  \nonumber \\
    &\leq c \alpha^{1.5}\tau \mathbf{e}_{t,i,s} + noise
\end{align}

but still need to deal with past noise and current iterates being a function of them







}
\end{proof}






% The $\tfrac{\sqrt{k} + \sqrt{\log(…)}}{\sqrt{b}}$ error is unavoidable.
% The log term will be very small . 
% For any $s$, note that $\mathbf{e}_{T,M+1,s}\coloneqq \mathbf{B}_{T,M+1,s}\mathbf{w}_{T,M+1,s} - \mathbf{B}_\ast \mathbf{w}_{\ast,M+1}$ can be written as:
% \begin{align}
% \mathbf{e}_{T,M+1,s} = \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top \mathbf{e}_{T,M+1,s} + (\mathbf{I}_k - \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top) \mathbf{e}_{T,M+1,s} 
% \end{align}
% where
% \begin{align}
%  (\mathbf{I}_k - \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top) \mathbf{e}_{T,M+1,s} &=  (\mathbf{I}_k - \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top) \mathbf{B}_{\ast} \mathbf{w}_{\ast,M+1} &\leq \dist_T \|\mathbf{w}_{\ast,M+1}\|_2. 
% \end{align}
% by the Cauchy-Schwarz Inequality and the fact that $\|(\mathbf{I}_k - \mathbf{\hat{B}}_T \mathbf{\hat{B}}_T^\top) \mathbf{B}_{\ast}\|_2 = \dist_T$. On the other hand,

% $\delta+ <= (delta  + dist) * (b+log)/k(1  + alpha^2\tau) + alpha^2\tau * delta + (1 - alpha^2) dist$

% \begin{align}
%     &\leq  \delta (1  + \alpha^2\tau) (b+\log)/k  +  \dist ( (1  + \alpha^2\tau)(b+\log)/k  + 1 - \alpha^2) \nonumber \\
%     &\leq \delta' ((1  + \alpha^2\tau) (b+\log)/k )^2 + +  \dist ( (1  + \alpha^2\tau)(b+\log)/k  + 1 - \alpha^2)(1 + ((1  + \alpha^2\tau) (b+\log)/k ) )  \nonumber \\
%     &\vdots \nonumber \\
%     &= \delta_0 ()^s + \dist \sum_{r=1}^s ((1  + \alpha^2\tau) (b+\log)/k)^{s-r} \nonumber \\
%     &\leq  \delta_0 ()^s + c \dist
% \end{align}

\begin{lemma}
For all $r\leq s$,
\begin{align}
\|  \mathbf{B}_{t,i,s}^\top  \mathbf{N}_{t,i,r}\| &\leq \tfrac{\sqrt{k}+ \sqrt{\log()}}{\sqrt{b}}
\end{align}
with high probability
\end{lemma}

\begin{proof}
We know 
\begin{align}
    \|  \mathbf{B}_{t,i,s-1}^\top  \mathbf{N}_{t,i,r}\| &\leq \tfrac{\sqrt{k}+ \sqrt{\log()}}{\sqrt{b}}
\end{align} whp
for all $r\leq s-1$.



We have
\begin{align}
    \|  \mathbf{B}_{t,i,s}^\top  \mathbf{N}_{t,i,r}\| &\leq \|  \mathbf{B}_{t,i,s-1}^\top  \mathbf{N}_{t,i,r}\| 
\end{align}






\end{proof}








\begin{lemma}
Distance does not get worse locally.
\end{lemma}

\begin{proof}

\begin{align}
   \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t,i,s+1}\|_2 &=  \|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_{T,M+1,s} (\mathbf{I}_k - \alpha \mathbf{w}_{T,M+1,s}\mathbf{w}_{T,M+1,s}^\top) \|_2\nonumber \\
   &\leq \|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_{t,i,s} \|_2 \nonumber  \\
   &\leq \|\mathbf{B}_{\ast,\perp}^\top \mathbf{B}_{t} \|_2
\end{align}
Thus
\begin{align}
    \dist_{t,s} \leq \frac{\|\mathbf{B}_{t}\|_2 }{\sigma_{\min}(\mathbf{B}_{t,i,s})} \dist_{t} \leq \sqrt{\tfrac{1+ \alpha^2 \tau c_{\del}}{1 -  c\alpha^2 \tau c_{\del}}} \dist_{t} 
\end{align}

With finite samples, we have:

just need to control:

\begin{align}
    
\end{align}





\end{proof}




% TODO:
% - cosine similarity of the features
% - plots for cifar10 dirichlet, cifar100 dirichlet, and emnist dirichlet
% - finite-sample results
% - poster
% % - rebuttal

% Takeaways:

% - dsgd change reps more in homogeneous data case





% \begin{proposition}[Distributed GD lower bound]
% Suppose we are in the setting described above and $k > 1$. Let $\mathbf{B}_0$ and $\mathbf{B}_T$ be the representation initialization and $T$-th iterate of Distributed GD, respectively.  Then for any set of ground-truth heads $\{\mathbf{w}_{\ast,i}\}_{i=1}^n$, $T>0$, $\delta_0 \in (0,1/2]$ and $\mathbf{B}_0\in\mathbb{R}^{d\times k}$, there exists $\mathbf{B}_\ast\in \mathcal{O}^{d \times k}$ such that $\dist(\mathbf{B}_0, \mathbf{B}_\ast) = \delta_0$ and $\dist(\mathbf{B}_T(\mathbf{B}_0,\mathbf{B}_\ast), \mathbf{B}_\ast) \geq \delta_0$, where $\mathbf{B}_T(\mathbf{B}_0,\mathbf{B}_\ast)$ is the result of running Distributed Gradient Descent (D-GD) with initialization $\mathbf{B}_0$ on the system with ground-truth representation $\mathbf{B}_\ast$.
% % \begin{enumerate}
% % \item $\dist(\mathbf{B}_T, \mathbf{B}_\ast) > \epsilon$, or
% % \item $\exists \; \mathbf{B}_\ast' \in \mathcal{O}^{d\times k}$ such that $\dist(\mathbf{B}_T, \mathbf{B}_\ast') > \min(2 \delta_0,1) -\epsilon$.
% % \end{enumerate}
% \end{proposition}

\subsection{Proof of Proposition \ref{prop:dgd}.}

\begin{proof}
Let $\mathbf{\bar{w}}_\ast \coloneqq \tfrac{1}{M}\sum_{i=1}^M \mathbf{w}_{\ast,i}$. 
Note that for D-GD the global update for the representation is 
\begin{align}
    \mathbf{B}_{t+1} = \mathbf{B}_t - \frac{\alpha}{M}\sum_{i=1}^M \nabla_{\mathbf{B}} f_i(\mathbf{B}_t, \mathbf{w}_t) = \mathbf{B}_t - \alpha (\mathbf{B}_t \mathbf{w}_t -\mathbf{B}_\ast \mathbf{\bar{w}}_{\ast}) \mathbf{w}_t^\top,
\end{align}
and similarly, the update for the head is $\mathbf{w}_{t+1} = \mathbf{w}_t - \alpha\mathbf{B}_t^\top(\mathbf{B}_t\mathbf{w}_t - \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast})$. Thus, the behavior of D-GD is invariant for all settings with ground-truth representation $\mathbf{B}_{\ast}'$ and average ground-truth head $\mathbf{w}_\ast'$ satisfying $\mathbf{B}_\ast' \mathbf{\bar{w}}_\ast' = \mathbf{B}_\ast \mathbf{\bar{w}}_\ast$.


Suppose $\dist(\mathbf{B}_T(\mathbf{B}_0,\mathbf{B}_\ast), \mathbf{B}_\ast) < \delta_0$ for some such $\mathbf{B}_\ast$. There exists $\mathbf{B}_\ast'\in \mathcal{O}^{d\times k}$ such that $\dist(\mathbf{B}_0,\mathbf{B}_\ast')$ and $\dist(\mathbf{B}_\ast,\mathbf{B}_\ast')\geq 2 \delta_0$ such that $\mathbf{B}_\ast \mathbf{\bar{w}}_\ast = \mathbf{B}_\ast' \mathbf{\bar{w}}_\ast $. Since behavior of Distributed GD depends only on the product $\mathbf{B}_\ast \mathbf{\bar{w}}_\ast$ and not the factors $\mathbf{B}_\ast$ and $\mathbf{\bar{w}}_\ast$, $\mathbf{B}_T(\mathbf{B}_0,\mathbf{B}_\ast) = \mathbf{B}_T(\mathbf{B}_0,\mathbf{B}_\ast')$. Using this equality with the triangle inequality yields
\begin{align}
    \dist(\mathbf{B}_T(\mathbf{B}_0,\mathbf{B}_\ast'), \mathbf{B}_\ast'  ) = \dist(\mathbf{B}_T(\mathbf{B}_0,\mathbf{B}_\ast), \mathbf{B}_\ast'  ) &\geq \dist( \mathbf{B}_\ast,  \mathbf{B}_\ast') - \dist(\mathbf{B}_T(\mathbf{B}_0,\mathbf{B}_\ast), \mathbf{B}_\ast  ) \nonumber \\
    &\geq 2 \delta_0 - \delta_0 \geq \delta_0 \nonumber
\end{align}
\end{proof}





==> App_Finite_A2.tex <==


\begin{lemma} \label{lem:a2fs}
$A_2(t+1)$
\end{lemma}

\begin{proof}
   We argue similarly as in Lemma \ref{lem:a2}. Let $\mathbf{\hat{G}}_{t} \coloneqq \tfrac{1}{\alpha}(\mathbf{B}_{t} - \mathbf{B}_{t+1})= 
   \tfrac{1}{M}\sum_{i=1}^M\sum_{s=0}^{\tau-1}(\mathbf{\Sigma}_{t,i,s} \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top + \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top)$ and 
    $\mathbf{N}_{t} \coloneqq \mathbf{G}_{t}-\mathbf{\hat{G}}_{t} = \tfrac{1}{M}\sum_{i=1}^M\sum_{s=0}^{\tau-1} (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top - \tfrac{1}{b}\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top$.
    We have 
    \begin{align}
        \del_{t,i,s+1} &= \del_{t}  + \alpha^2 \mathbf{B}_{t}^\top \mathbf{\hat{G}}_{t} +\alpha^2 \mathbf{\hat{G}}_{t}^\top \mathbf{B}_{t} - \alpha^3 \mathbf{\hat{G}}_{t}^\top \mathbf{\hat{G}}_{t} \nonumber \\  %\\
        &= \del_{t}  + \alpha^2 \mathbf{B}_{t}^\top \mathbf{{G}}_{t} +\alpha^2 \mathbf{{G}}_{t}^\top \mathbf{B}_{t} - \alpha^3 \mathbf{{G}}_{t}^\top \mathbf{{G}}_{t} \nonumber \\
        &\quad - \alpha^2 \mathbf{{B}}_{t}^\top \mathbf{N}_{t} - \alpha^2 \mathbf{N}_{t}^\top\mathbf{{B}}_{t}  - \alpha^3 \mathbf{N}_{t}^\top \mathbf{G}_{t} +\alpha^3 \mathbf{\hat{G}}_{t}^\top \mathbf{N}_{t}
        % &= \del_{t,i,s}  + \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{{G}}_{t,i,s} +\alpha^2 \mathbf{{G}}_{t,i,s}^\top \mathbf{B}_{t,i,s} - \alpha^3 \mathbf{{G}}_{t,i,s}^\top \mathbf{{G}}_{t,i,s} \nonumber  \\
        % &\quad - \alpha^2 \mathbf{B}_{t,i,s}^\top \mathbf{{N}}_{t,i,s} -\alpha^2 \mathbf{{N}}_{t,i,s}^\top \mathbf{B}_{t,i,s} + \alpha^3 \mathbf{{G}}_{t,i,s}^\top \mathbf{{N}}_{t,i,s} + \alpha^3 \mathbf{{N}}_{t,i,s}^\top \mathbf{\hat{G}}_{t,i,s} 
    \end{align}
We can apply the same analysis from Lemma \ref{lem:a2} to bound the population terms. Doing so yields
\begin{align}
     \|\del_{t}  + &\alpha^2 \mathbf{B}_{t}^\top \mathbf{\hat{G}}_{t} +\alpha^2 \mathbf{\hat{G}}_{t}^\top \mathbf{B}_{t} - \alpha^3 \mathbf{\hat{G}}_{t}^\top \mathbf{\hat{G}}_{t} \| \nonumber \\
     &\leq (1 - \alpha^2 E_0 \tilde{\mu}^2_\ast )\|\del_t\|_2 + c\alpha^{6}\tau^{2} c_{\del}^2L_{\max}^2 + c \alpha^4 L_{\max}^4  + c (\alpha^{6} \tau^3 c_{\del}^2 L_{\max}^2   + \alpha^{4} \tau L_{\max}^4 )\dist_t \nonumber \\
     &\quad + c \alpha^6 \tau^2 c_{\del}^2 L_{\max}(L_{\max}+\sigma)\tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}} + c \alpha^4 \tau c_{\del} L_{\max}(L_{\max}+\sigma)\tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}} \label{berg11} 
\end{align}
where the terms in the last line come from the finite-sample bound on $\|\mathbf{w}_t - \alpha(\mathbf{I}_k + \del_t)\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}\|$ (Lemma \ref{lem:a1fs}) that results in a different bound on $\|\mathbf{h}_t\|$ in the proof of Lemma \ref{lem:a2}.

% To bound other noises, 







% -----

The remainder of the proof lies in bounding the noise terms. We have
\begin{align}
    \mathbf{B}_t^\top \mathbf{N}_{t} &= \frac{1}{M}\sum_{i=1}^M\sum_{s=0}^{\tau-1}  \mathbf{B}_t^\top(\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s}) \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top - \frac{1}{M} \sum_{i=1}^M\sum_{s=0}^{\tau-1}\tfrac{1}{b}\mathbf{B}_t^\top\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top \nonumber 
\end{align}
We first consider the second term. Make an epsilon-net argument

\begin{align}
   |\frac{1}{Mb} \sum_{i=1}^M\sum_{s=0}^{\tau-1} \mathbf{u}^\top \mathbf{B}_t^\top\mathbf{X}_{t,i,s}^\top\mathbf{z}_{t,i,s}\mathbf{w}_{t,i,s}^\top \mathbf{v}| &\leq  
\end{align}
with high probability, we have $\max_s \|\mathbf{w}_{t,i,s}\| \leq  c \sqrt{\alpha} L$. 

should be able to say that since the sub-exponential random variables are independent from the weights





------


We aim to write $\del_{t+1} = \tfrac{1}{2}(\mathbf{I}_k - \mathbf{P}_t)\del_t + \tfrac{1}{2}\del_t(\mathbf{I}_k - \mathbf{P}_t) + \mathbf{Z}_t$ for a positive definite matrix $\mathbf{P}_t$ and a perturbation matrix $\mathbf{Z}_t$. This will yield the inequality $\|\del_{t+1}\|_2 \leq (1 - \lambda_{\min}(\mathbf{P}_t))\|\del_{t}\|_2 + \|\mathbf{Z}_t\|_2$. Assuming $\lambda_{\min}(\mathbf{P}_t)$ and $\|\mathbf{Z}_t\|_2$ scale appropriately (defined later), this inequality combined with inductive hypothesis $A_3(t)$ will give the desired upper bound on $\|\del_{t+1}\|_2$. The proof therefore relies on showing the existence of appropriate $\mathbf{P}_t$ and $\mathbf{Z}_t$. 

First recall $\del_t \coloneqq \mathbf{I} - \alpha\mathbf{B}_t^\top \mathbf{B}_t$ and $\deld_t \coloneqq \mathbf{I}_d - \alpha \mathbf{B}_t \mathbf{B}_t^\top$. Let $\mathbf{G}_t \coloneqq \tfrac{1}{\alpha}(\mathbf{B}_t - \mathbf{B}_{t+1})$, i.e. $\mathbf{G}_t$ satisfies $\mathbf{B}_{t+1}= \mathbf{B}_t - \alpha \mathbf{G}_t$.
Then
\begin{align}
    \del_{t+1} &= \mathbf{I}_k - \alpha \mathbf{B}_{t+1}^\top \mathbf{B}_{t+1} =  \del_t + \alpha^2 \mathbf{B}_t^\top \mathbf{G}_t + \alpha^2 \mathbf{G}_t^\top \mathbf{B}_t - \alpha^3 \mathbf{G}_t^\top \mathbf{G}_t \label{del2}
\end{align}
The key is showing that $\alpha^2 \mathbf{B}_t^\top \mathbf{G}_t = -\tfrac{1}{2}\del_t \mathbf{P}_t + \mathbf{Z}_t'$ for appropriate $\mathbf{P}_t$ and $\mathbf{Z}_t'$. Then, by \eqref{del}, we will have $\del_{t+1} =  \tfrac{1}{2}(\mathbf{I}_k - \mathbf{P}_t)\del_t + \tfrac{1}{2}\del_t(\mathbf{I}_k - \mathbf{P}_t) + \mathbf{Z}_t $ as desired, where $\mathbf{Z}_t = \mathbf{Z}_t' + (\mathbf{Z}_t')^\top - \alpha^3 \mathbf{G}_t^\top \mathbf{G}_t$.




Notice that $\mathbf{G}_t$ is the average across clients of the sum of their local gradients on every local update. In particular, we have 
\begin{align}
    \mathbf{G}_t = (\mathbf{B}_{t}\mathbf{w}_{t}- \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t})\mathbf{w}_{t}^\top +\tfrac{1}{n}\sum_{i=1}^n \sum_{s = 1}^{\tau-1} (\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top 
\end{align}
We will unroll the first local update only. Namely, consider the local gradients {\em after} one local update. 
Expanding $\mathbf{B}_{t,i,1}$ and $\mathbf{w}_{t,i,1}$ yields
\begin{align}
  &\tfrac{1}{M}\sum_{i=1}^M (\mathbf{B}_{t,i,1}\mathbf{w}_{t,i,1}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,1}^\top \nonumber \\
  &= \tfrac{1}{M}\sum_{i=1}^M (\mathbf{B}_{t}\mathbf{w}_{t,i,1}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,1}^\top - \tfrac{\alpha}{M} \sum_{i=1}^M \mathbf{e}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top \nonumber \\
  &\quad - \tfrac{\alpha}{M} \sum_{i=1}^M (\mathbf{\Sigma}_{t,i,0} - \mathbf{I}_d ) \mathbf{e}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top - \tfrac{\alpha}{Mb} \sum_{i=1}^M \mathbf{X}_{t,i,0}^\top \mathbf{z}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top  \nonumber \\
  &= -\tfrac{1}{M}\sum_{i=1}^M \deld_t \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,1}^\top + \tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_{t}\del_t\mathbf{w}_{t}\mathbf{w}_{t,i,1}^\top + \tfrac{\alpha}{M}\sum_{i=1}^M \mathbf{B}_{t}\mathbf{B}_{t}^\top(\mathbf{I}_d- \mathbf{\Sigma}_{t,i,0})\mathbf{e}_{t,i,0}\mathbf{w}_{t,i,1}^\top  \nonumber  \\
  &\quad - \tfrac{\alpha}{Mb}\sum_{i=1}^M \mathbf{B}_{t}\mathbf{B}_{t}^\top \mathbf{X}_{t,i,0}^\top \mathbf{z}_{t,i,0} \mathbf{w}_{t,i,1}^\top  - \tfrac{\alpha}{M} \sum_{i=1}^M \mathbf{e}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top \nonumber \\
  &\quad - \tfrac{\alpha}{M} \sum_{i=1}^M (\mathbf{\Sigma}_{t,i,0} - \mathbf{I}_d ) \mathbf{e}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top - \tfrac{\alpha}{Mb} \sum_{i=1}^M \mathbf{X}_{t,i,0}^\top \mathbf{z}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top      \nonumber \\
  &= -\tfrac{\alpha}{M}\sum_{i=1}^M \deld_t \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t - \deld_t \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{w}_{t}^\top \del_t \nonumber \\
  &\quad - \tfrac{\alpha}{M}\sum_{i=1}^M \deld_t \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{e}_{t,i,0}^\top (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,0}) \mathbf{B}_t  -  \tfrac{\alpha}{Mb}\sum_{i=1}^M \deld_t \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} \mathbf{z}_{t,i,0}^\top \mathbf{X}_{t,i,0} \mathbf{B}_t \nonumber \\
  &\quad +  \mathbf{B}_{t}\del_t\mathbf{w}_{t}\mathbf{w}_{t}^\top \del_t + \alpha\mathbf{B}_{t}\del_t\mathbf{w}_{t}\mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \tfrac{\alpha}{M}\sum_{i=1}^M  \mathbf{B}_{t}\del_t\mathbf{w}_{t} \mathbf{e}_{t,i,0}^\top (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,0})\mathbf{B}_t \nonumber \\
  &\quad + \tfrac{\alpha}{Mb}\sum_{i=1}^M  \mathbf{B}_{t}\del_t\mathbf{w}_{t} \mathbf{z}_{t,i,0}^\top  \mathbf{X}_{t,i,0}\mathbf{B}_t + \tfrac{\alpha}{M}\sum_{i=1}^M \mathbf{B}_{t}\mathbf{B}_{t}^\top(\mathbf{I}_d- \mathbf{\Sigma}_{t,i,0})\mathbf{e}_{t,i,0}\mathbf{w}_{t,i,1}^\top  \nonumber  \\
  &\quad - \tfrac{\alpha}{Mb}\sum_{i=1}^M \mathbf{B}_{t}\mathbf{B}_{t}^\top \mathbf{X}_{t,i,0}^\top \mathbf{z}_{t,i,0} \mathbf{w}_{t,i,1}^\top  - \tfrac{\alpha}{M} \sum_{i=1}^M \mathbf{e}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top \nonumber \\
  &\quad - \tfrac{\alpha}{M} \sum_{i=1}^M (\mathbf{\Sigma}_{t,i,0} - \mathbf{I}_d ) \mathbf{e}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top - \tfrac{\alpha}{Mb} \sum_{i=1}^M \mathbf{X}_{t,i,0}^\top \mathbf{z}_{t,i,0} \mathbf{w}_t^\top \mathbf{w}_{t,i,1} \mathbf{w}_{t,i,1}^\top      \nonumber 
\end{align}
Multiplying both sides by $\mathbf{B}_t^\top$ and using $\mathbf{B}_t^\top \deld_t = \del_t \mathbf{B}_t^\top$ yields
\begin{align}
    &\tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_t^\top(\mathbf{B}_{t,i,1}\mathbf{w}_{t,i,1}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,1}^\top \nonumber \\
    &= -\tfrac{\alpha}{M}\sum_{i=1}^M \del_t\mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \alpha\mathbf{B}_t^\top\mathbf{B}_{t}\del_t\mathbf{w}_{t}\mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  + \mathbf{Q}_t
\end{align}
where 
\begin{align}
   \| \mathbf{Q}_t \|_2 &\leq 2 c \|\del\|^2 \eta_\ast^2 + 2c\|\del\| L_{\max}(L_{\max}+\sigma)\tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}} \nonumber \\
   &\quad + L_{\max}(L_{\max}+\sigma) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}} + \alpha^2 L_{\max}^3( L_{\max} + (L_{\max}+\sigma)\tfrac{\sqrt{k} +\sqrt{\log()}}{\sqrt{Mb}}) \nonumber \\
   &= O(\|\del\|^2 L_{\max}^2 + L_{\max}(L_{\max}+\sigma)\tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}} + \alpha^2 L_{\max}^4 )
\end{align}
with probability at least $1 - $.
Thus, we have
\begin{align}
    \mathbf{B}_t^\top \mathbf{G}_t &= \mathbf{B}_t^\top(\mathbf{B}_{t}\mathbf{w}_{t}- \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t})\mathbf{w}_{t}^\top +\tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_t^\top(\mathbf{B}_{t,i,1}\mathbf{w}_{t,i,1}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,1}^\top \nonumber \\
    &\quad +\tfrac{1}{M}\sum_{i=1}^M \sum_{s = 2}^{\tau-1} \mathbf{B}_t^\top(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top \nonumber \\
    &= -\tfrac{\alpha}{M}\sum_{i=1}^M \del_t\mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \underbrace{\mathbf{B}_t^\top(\mathbf{B}_{t}\mathbf{w}_{t}- \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t})\mathbf{w}_{t}^\top  + \alpha\mathbf{B}_t^\top\mathbf{B}_{t}\del_t\mathbf{w}_{t}\mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t}_{=:\mathbf{E}_t}  \nonumber \\
    &\quad + \mathbf{Q}_t +\underbrace{\tfrac{1}{M}\sum_{i=1}^M \sum_{s = 2}^{\tau-1} \mathbf{B}_t^\top(\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top}_{=:\mathbf{E}_t'} \label{78}
\end{align}
 As in the proof of Lemma \ref{lem:a2}, we deal with $\mathbf{E}$ by using the fact that $\mathbf{w}_t$ is close to a matrix times $\mathbf{\bar{w}}_{\ast,t}$. This will allow us to subsume the dominant term from $\mathbf{E}$ into the negative term in \eqref{78}. 
In particular, note that by $\bar{A}_1(t)$, we have $\mathbf{w}_t = \alpha \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t} + \alpha\del_{t} \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t} + \mathbf{h}_t$, where $\|\mathbf{h}_t\|_2 \leq c\alpha^{0.5} (L_{\max}+ \sigma) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{Mb}}  +  c \alpha^{2.5}\tau L_{\max}^3 +  c\alpha^{2.5}\tau c_{\del}(L_{\max} + \sigma ) \tfrac{\sqrt{k}+\sqrt{\log()}}{\sqrt{{Mb}}} + c \alpha^{4.5}\tau^2 L_{\max} c_{\del}^2$. 

$ \equiv c\alpha^{0.5}(L_{\max}+ \sigma) \delta +  c \alpha^{2.5}\tau L_{\max}^3 + c \alpha^{0.5}L\|\del\|^2$.
This implies that
\begin{align}
    \mathbf{B}_t^\top(\mathbf{B}_{t}\mathbf{w}_{t}- \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}) &= \mathbf{B}_t^\top(\alpha \mathbf{B}_{t}\mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}  - \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}) + \alpha \del_t\mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} + \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \nonumber\\
    % &\quad + \alpha \mathbf{B}_t^\top \mathbf{B}_{t}(\mathbf{B}_{t-1}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t-1} -\mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t})+  \alpha \mathbf{B}_t^\top \mathbf{B}_{t}(\del_{t-1}\mathbf{B}_{t-1}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t-1} -\del_{t}\mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}) \nonumber\\
    &= -\del_t \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} + \alpha \del_t\mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} + \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \nonumber\\
    % &\quad + \alpha \mathbf{B}_t^\top \mathbf{B}_{t}(\mathbf{B}_{t-1}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t-1} -\mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t})+  \alpha \mathbf{B}_t^\top \mathbf{B}_{t}(\del_{t-1}\mathbf{B}_{t-1}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t-1} -\del_{t}\mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}) \nonumber\\
    &= -\del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t} + \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} %+ \mathbf{\tilde{e}}_{t} 
\end{align}
% where $\mathbf{\tilde{e}}_{t} \coloneqq  \alpha \mathbf{B}_t^\top \mathbf{B}_{t}(\mathbf{B}_{t-1}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t-1} -\mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t})+  \alpha \mathbf{B}_t^\top \mathbf{B}_{t}(\del_{t-1}\mathbf{B}_{t-1}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t-1} -\del_{t}\mathbf{B}_{t}^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t})$. 
which leads to 
\begin{align}
  \mathbf{E}_t &:= \mathbf{B}_t^\top(\mathbf{B}_{t}\mathbf{w}_{t}- \mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t})\mathbf{w}_{t}^\top  + \alpha\mathbf{B}_t^\top\mathbf{B}_{t}\del_t\mathbf{w}_{t}\mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \nonumber \\
   &=  -\del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{{w}}_{t}^\top + \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \mathbf{{w}}_{t}^\top + \alpha \mathbf{B}_t^\top\mathbf{B}_t\del_t \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \nonumber  \\
    &= -\del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{{w}}_{t}^\top + \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \mathbf{{w}}_{t}^\top  -\del_t^2 \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  + \del_t \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \nonumber \\
    &= -\del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{{w}}_{t}^\top + \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \mathbf{{w}}_{t}^\top  -\del_t^2 \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  \nonumber \\
    &\quad +  \del_t(\alpha\del_{t} \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}+\mathbf{h}_t)  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \alpha \del_t \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t. \label{above2}
\end{align} 
We can subsume the last term in \eqref{above2} into the negative term in \eqref{78} by completing a square. In particular, 
\begin{align}
   &-\tfrac{\alpha}{M}\sum_{i=1}^M \del_t\mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \mathbf{E} \nonumber \\
   &= -\tfrac{\alpha}{M}\sum_{i=1}^M \del_t\mathbf{B}_t^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top \mathbf{B}_\ast^\top \mathbf{B}_t-\del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{{w}}_{t}^\top + \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \mathbf{{w}}_{t}^\top  -\del_t^2 \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  \nonumber \\
    &\quad +  \del_t(\alpha\del_{t} \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}+\mathbf{h}_t)  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \alpha \del_t \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \nonumber \\
    &= - \alpha \del_t \mathbf{B}_t^\top \mathbf{B}_\ast \tfrac{1}{M}\sum_{i=1}^M (\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})(\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})^\top\mathbf{B}_\ast^\top \mathbf{B}_t - \del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{{w}}_{t}^\top \nonumber \\
    &\quad  + \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \mathbf{{w}}_{t}^\top  -\del_t^2 \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  +  \del_t(\alpha\del_{t} \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}+\mathbf{h}_t)  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  
\end{align}
meaning that 
% ----
% Note that all terms involving a $\del_t$ scale with $\alpha^4$, with the exception of one term (the term in the last line). With slight abuse of notation, we use $\mathcal{O}(*)$ notation to denote a matrix whose spectral norm scales as $\mathcal{O}(*)$. We have
% \begin{align}
%     \mathbf{E}_1 &= \alpha \del_t \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t + \mathcal{O}(\alpha^4 \tau^2 c_{\del}^2 L_{\max} + \alpha^2 \tau L_{\max}^4 ) \label{36}
% \end{align}
% The first term term can be subsumed by completing a square as follows.
% Combining \eqref{61}, \eqref{split}, and  \eqref{36} yields
\begin{align}
    \mathbf{B}_t^\top \mathbf{G}_t 
    % &= - \alpha \del_t \mathbf{B}_t^\top \mathbf{B}_\ast \tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top \mathbf{B}_t + \mathbf{E}_1 -  \mathbf{E}_2 +\mathbf{E}_3 + \mathbf{E}_4 \nonumber \\
    % &= - \alpha \del_t \mathbf{B}_t^\top \mathbf{B}_\ast \tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,t,i}\mathbf{w}_{\ast,t,i}^\top\mathbf{B}_\ast^\top \mathbf{B}_t  + \alpha \del_t \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  \nonumber \\
    % &\quad -  \mathbf{E}_2 +\mathbf{E}_3 + \mathbf{E}_4  +  \mathcal{O}(\alpha^4 \tau^2 c_{\del}^2 L_{\max} + \alpha^2 \tau L_{\max}^4 )  \nonumber \\
    % &= - \alpha \del_t \mathbf{B}_t^\top \mathbf{B}_\ast \tfrac{1}{n}\sum_{i=1}^n (\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})(\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})^\top\mathbf{B}_\ast^\top \mathbf{B}_t  \nonumber \\
    % &\quad -  \mathbf{E}_2 +\mathbf{E}_3 + \mathbf{E}_4  +  \mathcal{O}(\alpha^4 \tau^2 c_{\del}^2 L_{\max}^2 + \alpha^2 \tau L_{\max}^4 )  \nonumber \\
    &=  - \tfrac{1}{2\alpha^2} \del_t \mathbf{P}_t + \tfrac{1}{\alpha^2}\mathbf{Z}'_t
\end{align}
where $\mathbf{P}_t = 2\alpha^3\mathbf{B}_t^\top \mathbf{B}_\ast \tfrac{1}{n}\sum_{i=1}^n (\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})(\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})^\top\mathbf{B}_\ast^\top \mathbf{B}_t$ and 
\begin{align}
   \mathbf{Z}'_t &:= - \alpha^2 \del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{{w}}_{t}^\top  + \alpha^2 \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \mathbf{{w}}_{t}^\top -\alpha^2\del_t^2 \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \nonumber \\
    &\quad   +  \alpha^2\del_t(\alpha\del_{t} \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}+\mathbf{h}_t)  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t +  \alpha^2\mathbf{Q}_t  -  \alpha^2\mathbf{E}_t'  
\end{align}
we have performed the desired decomposition; it remains to show that $\lambda_{\min}(\mathbf{P}_t)$ and $\|\mathbf{Z}'_t\|_2$ scale appropriately.
 First we lower bound $\lambda_{\min}(\mathbf{P}_t)$, identically to as in Lemma \ref{lem:a2}.
 \begin{align}
     \lambda_{\min}(\mathbf{P}_t) &= \lambda_{\min}\left(2\alpha^3\mathbf{B}_t^\top \mathbf{B}_\ast \tfrac{1}{n}\sum_{i=1}^n (\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})(\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})^\top\mathbf{B}_\ast^\top \mathbf{B}_t\right) \nonumber \\
    %  &\geq 2 \alpha^3 \sigma_{\min}(\mathbf{B}_t^\top \mathbf{B}_\ast)^2 \lambda_{\min}\left(\tfrac{1}{n}\sum_{i=1}^n (\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})(\mathbf{w}_{\ast,t,i} - \mathbf{\bar{w}}_{\ast,t})^\top\right) \nonumber \\
     &\geq \alpha^2 E_0 \tilde{\mu}_\ast^2
 \end{align}
 Next we upper bound $\|\mathbf{Z}'_t\|_2$. We already have an upper bound on $\|\mathbf{Q}_t\|$. We next bound the rest of the terms in $\mathbf{Z}'_t$ besides $\mathbf{E}'_{t}$. We have
% $ c\alpha^{0.5}(L_{\max}+ \sigma) \delta +  c \alpha^{2.5}\tau L_{\max}^3 + c \alpha^{0.5}L\|\del\|^2$
 \begin{align}
 &  \|\alpha^2 \mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \mathbf{{w}}_{t}^\top- \alpha^2 \del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{{w}}_{t}^\top  -\alpha^2\del_t^2 \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t   +  \alpha^2\del_t(\alpha\del_{t} \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t}+\mathbf{h}_t)  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  \| \nonumber \\
     &\leq  2\alpha^2 L (L+\sigma) \delta + 2 \alpha^4 \tau L^4 + 5\alpha^2 L^2 \|\del_t\|^2 
 \end{align}
%  start by upper bounding $\|\alpha^2 \mathbf{E}_2\|_2$ and $\|\alpha^2\mathbf{E}_3\|_2$. We have
%  \begin{align}
%      \|\alpha^2\mathbf{E}_2\|_2 &\leq c \alpha^4  L_{\max}^4 + c \alpha^6 \tau c_{\del} L_{\max}^4  \leq c' \alpha^4  L_{\max}^4  \nonumber \\
%     %  \alpha^4 c(1+\tilde{c})c_2^2 L_{\max}^3 \eta_\ast + \alpha^4 c (1+\tilde{c})c_2^3 L_\ast^2 \eta_\ast^2\|\del_t\|_2 \nonumber \\
%      \|\alpha^2\mathbf{E}_3\|_2 &\leq \alpha^6 \tau^2 c_{\del}^2 L_{\max}^2 \nonumber  %  c(1+\tilde{c}) c_2^2\eta_\ast^2 \|\del_t\|_2^2 \nonumber
%  \end{align}
% Next we upper bound the remaining terms in $\mathbf{Z}'_t$ besides $\mathbf{E}_{4}$. We have
% \begin{align}
%     \Big\|&-\alpha^2\del_t^2 \mathbf{B}_t^\top\mathbf{B}_\ast\mathbf{\bar{w}}_{\ast,t}\mathbf{{w}}_{t}^\top + \alpha^2\mathbf{B}_t^\top \mathbf{B}_{t}\mathbf{h}_{t} \mathbf{{w}}_{t}^\top +\alpha^2 \mathbf{\tilde{e}}_{t} \mathbf{w}_t^\top -\alpha^2\del_t^2 \mathbf{w}_{t}  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  \nonumber \\
%     &\quad +  \alpha^2\del_t(\alpha\del_{t-1} \mathbf{B}_{t-1}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t-1}+\mathbf{h}_t)  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t  + \alpha^3 \del_t (\mathbf{B}_{t-1}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t-1}- \mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{\bar{w}}_{\ast,t})  \mathbf{\bar{w}}_{\ast,t}^\top \mathbf{B}_\ast^\top \mathbf{B}_t \Big\|_2 \nonumber \\
%     &\leq \alpha^6 c (1+\tilde{c})c_2 c_3^2 \tilde{\kappa}_\ast^2 L_\ast^2 \eta_\ast^4 \tau  + \alpha^4 c (1+\tilde{c})c_2^3  \eta_\ast (L_\ast^2 \eta_\ast + \tilde{\kappa}_\ast^{-4} L_{\max} \eta_\ast^2)
% \end{align}
%** assuming \tilde{e} is dominated, which it is, and $\|\mathbf{\bar{w}}_{\ast,t}- \mathbf{\bar{w}}_{\ast,t-1}\|_2$


Now we bound $\|\alpha^2\mathbf{E}'_t\|_2$. Recall that $\mathbf{E}_t'$ is the sum of local gradients across all clients and all local updates beyond the first local update. We show that these gradients are sufficiently small such that $\|\del_{t+1}\|_2$ cannot grow beyond the desired threshold.
% \begin{align}
%     \|\alpha^2\mathbf{E}_4\|_2 &=  \alpha^2\left\| \mathbf{B}_t^\top\tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} (\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top \right\|_2  \nonumber \\
%     &\leq  \alpha^2\left\| \tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} (-\mathbf{B}_t^\top\deld_{t,i,s} + \alpha \mathbf{B}_t^\top\deld_{t,i,s}\mathbf{B}_{t,i,s} \mathbf{B}_{t,i,s}^\top) \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top \right\|_2 +  c \alpha^4 \tau \eta_\ast (L_\ast^2 \eta_\ast + \kappa_{\ast}^{-4}L_{\max}\eta_\ast^2 ) \nonumber \\
%     &\leq \alpha^2\left\| \tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} -\mathbf{B}_t^\top\deld_{t,i,s}^2 \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top \right\|_2 +  c \alpha^4 \tau L_\ast^4(L_\ast^2 \eta_\ast + \kappa_{\ast}^{-4}L_{\max}\eta_\ast^2 )  \nonumber \\
%     &\leq   \alpha^2\left\| \tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} -\mathbf{B}_{t,i,2}^\top\deld_{t,i,s}^2 \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top \right\|_2  + (1+\tilde{c})\alpha^4 L_\ast^2  +  c \alpha^4 \tau L_\ast^4(L_\ast^2 \eta_\ast + \kappa_{\ast}^{-4}L_{\max}\eta_\ast^2 )    \nonumber \\
%      &\leq   \alpha^2\left\| \tfrac{1}{n}\sum_{i=1}^n \sum_{s = 3}^{\tau-1} -\mathbf{B}_{t,i,2}^\top\deld_{t,i,s}^2 \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top \right\|_2 + \alpha^2\left\| \tfrac{1}{n}\sum_{i=1}^n  -\del_{t,i,2}^2\mathbf{B}_{t,i,2}^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,2}^\top \right\|_2  + (1+\tilde{c})\alpha^2 L_\ast^2  \nonumber\\
%      &\quad +  c \alpha^4 \tau L_\ast^4(L_\ast^2 \eta_\ast + \kappa_{\ast}^{-4}L_{\max}\eta_\ast^2 )    \nonumber \\
%      &\leq   \alpha^2\left\| \tfrac{1}{n}\sum_{i=1}^n \sum_{s = 4}^{\tau-1} -\mathbf{B}_{t,i,3}^\top\deld_{t,i,s}^2 \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top \right\|_2 + \alpha^2\left\| \tfrac{1}{n}\sum_{i=1}^n  -\del_{t,i,3}^2\mathbf{B}_{t,i,3}^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,3}^\top \right\|_2 +  \nonumber\\
%      &\quad  + \alpha^2\left\| \tfrac{1}{n}\sum_{i=1}^n  -\del_{t,i,2}^2\mathbf{B}_{t,i,2}^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,2}^\top \right\|_2  + (1+\tilde{c})\alpha^2 L_\ast^2 +  c \alpha^4 \tau L_\ast^4(L_\ast^2 \eta_\ast + \kappa_{\ast}^{-4}L_{\max}\eta_\ast^2 )    \nonumber \\
%      &\quad \vdots \nonumber \\
%     &\leq c\alpha^6 \tau^2   \tilde{\kappa}_{\ast}^2 L_\ast^6  +  c \alpha^4 \tau L_\ast^4(L_\ast^2 \eta_\ast + \kappa_{\ast}^{-4}L_{\max}\eta_\ast^2 ) 
% \end{align}
% % using $\mathbf{w}_{t,i,s} \approx \alpha(\mathbf{I}+\elta_{t,i,s-1})\mathbf{B}_{t,i,s-1}^\top \mathbf{B}_\ast\mathbf{{w}}_{\ast,t,i} $.
% Combining these bounds, we obtain
% \begin{align}
%     \|\mathbf{Z}'_t\|_2 &\leq  c\alpha^6 \tau^2   \tilde{\kappa}_{\ast}^2 L_\ast^6  +  c \alpha^4 \tau L_\ast^4
% \end{align}

% It can be shown that $\|\mathbf{G}_t^\top \mathbf{G}_t\|_2 \leq c''\alpha^3  \tilde{\kappa}_{\ast}^2 L_\ast^6\tau^2$ for an absolute constant $c$.
% Thus we have
% \begin{align}
%     \|\del_{t+1}\|_2 &\leq (1 - c \alpha^2 \tilde{\mu_\ast}^2) \|\del_t\|_2 + c'  \alpha^4  \tau L_\ast^4 + c'' \alpha^6 \tilde{\kappa}_{\ast}^2L_\ast^6\tau^2
% \end{align}
% which implies that if $\|\del_{t}\|_2 \leq c_3 \alpha^2 \tau \tilde{\kappa}_{\ast}^2 L_\ast^2$ for some absolute constant $c_3$, then  $\|\del_{t+1}\|_2 \leq c_3 \alpha^2 \tau \tilde{\kappa}_{\ast}^2 L_\ast^2$, noting that $\alpha \leq c \tilde{\kappa}_{\ast}\tfrac{L_\ast}{\sqrt{\tau}}$.


% -----

% Update:






% First note that 
% \begin{align}
%     \|\mathbf{B}_{t,i,s+1}\mathbf{w}_{t,i,s+1} -\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\|_2 &\leq (\alpha^2 (\tau^x + L_{\max}))^s + \dist_{t,i,s} (1 - \alpha^2 \|\mathbf{w}_{\ast,t,i}\|_2^2)^s
% \end{align}
% Also, 
% \begin{align}
%     \|\mathbf{B}_{t,i,2}\mathbf{w}_{t,i,2} -\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\|_2 &=  \|\alpha\mathbf{B}_{t,i,2}\mathbf{B}_{t,i,1}^\top \mathbf{B}_\ast\mathbf{w}_{\ast,t,i} -\mathbf{B}_\ast \mathbf{w}_{\ast,t,i} + \mathbf{B}_{t,i,2} \del_{t,i,1}\mathbf{w}_{t,i,1}\|_2 \nonumber \\
%     % &\leq {  \|\deld_{t,i,1}(\mathbf{B}_{t,i,1}\mathbf{w}_{t,i,1}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) \|_2   +  \alpha^2 L_{\max}^2(1+\|\del_t\|_2)\|\mathbf{B}_{t,i,1}\mathbf{w}_{t,i,1} -\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\|_2 }  \nonumber \\
%     % &\leq { c\|\deld_{t,i,1}(\mathbf{B}_{t,i,1}\mathbf{w}_{t,i,1}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) \|_2  }\nonumber  %\\ 
%     &\leq \|(\deld_{t,i,1} - \alpha^2\|\mathbf{w}_{\ast,t,i}\|_2^2\mathbf{I}_d + \alpha^4 \|\mathbf{w}_{\ast,t,i}\|_2^2  c_{\del} \tau^x \mathbf{I}_d )(\mathbf{B}_{t,i,1}\mathbf{w}_{t,i,1}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) \|_2  \nonumber %\\
%     % &\leq  
%     % &\leq \|\deld_{t,i,1}(\mathbf{B}_{t,i,1}\mathbf{w}_{t,i,1}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) \|_2 + \alpha^2 L_{\max}^3 (1+\|\del_t\|_2) \nonumber \\
%     % &= \|\deld_{t,i,1}(\alpha\mathbf{B}_{t,i,1}\mathbf{B}_{t}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) + \deld_{t,i,1}\mathbf{B}_{t,i,1}\del_t \mathbf{w}_{t}  \|_2 + \alpha^2 L_{\max}^3 (1+\|\del_t\|_2)  \nonumber \\
%     % &\leq \|\deld_{t,i,1}\deld_t(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) \|_2 + \alpha^2L_{\max}^3( 1 + \|\del_t\|_2) + \alpha^2 L_{\max}^3 (1+\|\del_t\|_2)    \nonumber %\\
%     % &\leq \|\deld_{t,i,1}\deld_{t}(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) \|_2 + 2\alpha^2 L_{\max}^2 (1+\|\del_t\|_2) \nonumber %\\
%     % &\leq \|\del_t\|_2 L_{\max} +  \dist_t + 2\alpha^2 L_{\max}^2 (1+\|\del_t\|_2) 
% \end{align}
% Let $\mathbf{C}_{t,i,s}\coloneqq \deld_{t,i,s} - \alpha^2\|\mathbf{w}_{\ast,t,i}\|_2^2\mathbf{I}_d + \alpha^4 \|\mathbf{w}_{\ast,t,i}\|_2^2  c_{\del} \tau^x \mathbf{I}_d$.
% Similarly,
% \begin{align}
%     \|\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} -\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\|_2 &\leq \|\mathbf{C}_{t,i,s-1}\dots\mathbf{C}_{t,i,1}\mathbf{C}_t(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) \|_2    \nonumber \\
%     &\leq \|\mathbf{C}_{t,i,s-1}\dots\mathbf{C}_{t,i,1}\mathbf{C}_t(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_{\ast,t}\mathbf{w}_{\ast,t,i}) \|_2 +  \|\mathbf{C}_{t,i,s-1}\dots\mathbf{C}_{t,i,1}\mathbf{C}_t\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i} \|_2  \nonumber \\
%     &\leq \|\mathbf{C}_{t,i,s-1}\dots\mathbf{C}_{t,i,1}\alpha^2 (\|\mathbf{w}_{\ast,i}\|_2^2 + c_{\del}\tau^x)(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_{\ast,t}\mathbf{w}_{\ast,t,i}) \|_2 \nonumber \\
%     &\quad +  \|\mathbf{C}_{t,i,s-1}\dots\mathbf{C}_{t,i,1}\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i} \|_2  \nonumber \\
%     &\leq \|\mathbf{C}_{t,i,s-1}\dots\alpha^2(\|\mathbf{w}_{\ast,i}\|_2^2 +  + c_{\del}\tau^x  )\alpha^2 (\|\mathbf{w}_{\ast,i}\|_2^2 + c_{\del}\tau^x)(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_{\ast,t}\mathbf{w}_{\ast,t,i}) \|_2 \nonumber \\
%     &\quad +  \|\mathbf{C}_{t,i,s-1}\dots\mathbf{C}_{t,i,1}(1 - \alpha^2 \|\mathbf{w}_{\ast,i}\|_2)\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i} \|_2  \nonumber \\
%     &\quad \vdots \nonumber \\
%     &\leq \alpha^{2s}
%     % &\leq (1+\alpha^2L_{\max})^s\|\deld_{t,i,s-1}\dots\deld_{t,i,1}\deld_t(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_{\ast,t}\mathbf{w}_{\ast,t,i}) \|_2 \nonumber \\
%     % &\quad + (1+\alpha^2L_{\max})^s\|\deld_{t,i,s-1}\dots\deld_{t,i,1}\deld_t\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i}\|_2  \nonumber \\
%     % &\leq (1+\alpha^2L_{\max})^s (\alpha^2 \tau^x c_{\del}(1+\alpha^2L_{\max}))^{s-1} L_{\max} + (1+\alpha^2L_{\max})^s\|\deld_{t,i,s-1}\dots\deld_{t,i,1}\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i}\|_2  \nonumber \\
% \end{align}
% Note that we don't need to worry about $\deld_{t,i,s}\mathbf{B}_t$ having an extra error term growing with $\tau$ due to $(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s}\mathbf{\hat{B}}_{t,i,s}^\top)\mathbf{B}_t$  because $\mathbf{\hat{B}}_{t,i,s}$ is changing. We don't have to worry about this because the distance is

% \begin{align}
%     \|\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s} -\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\|_2 &\leq \|\deld_{t,i,s-1}\dots\deld_{t,i,1}\deld_t(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_\ast\mathbf{w}_{\ast,t,i}) \|_2    \nonumber \\
%     &\leq (1+\alpha^2L_{\max})^s\|\deld_{t,i,s-1}\dots\deld_{t,i,1}\deld_t(\mathbf{B}_{t}\mathbf{w}_{t}  - \mathbf{B}_{\ast,t}\mathbf{w}_{\ast,t,i}) \|_2 \nonumber \\
%     &\quad + (1+\alpha^2L_{\max})^s\|\deld_{t,i,s-1}\dots\deld_{t,i,1}\deld_t\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i}\|_2  \nonumber \\
%     &\leq (1+\alpha^2L_{\max})^s (\alpha^2 \tau^x c_{\del}(1+\alpha^2L_{\max}))^{s-1} L_{\max} + (1+\alpha^2L_{\max})^s\|\deld_{t,i,s-1}\dots\deld_{t,i,1}\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i}\|_2  \nonumber \\
% \end{align}
% {\color{blue}(no, use that $\alpha^2$ term is negative, get either 0 or $\alpha^4\tau^x$ term, both fine.)}
Recall that $\mathbf{E}_t' = \sum_{s=2}^{\tau-1} \mathbf{B}_t^\top \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top$. To bound this it is critical to control the evolution of $\mathbf{e}_{t,i,s}$. To do so, first let 
$\mathbf{\hat{B}}_{t,i,s},\mathbf{R}_{t,i,s}$ denote the QR-factorization of $\mathbf{B}_{t,i,s}$ and define $\tilde{\del}_{t,i,s-1} \coloneqq \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top - \alpha \mathbf{B}_{t,i,s-1}\mathbf{B}_{t,i,s-1}^\top$ and $\omega_{t,i,s-1} \coloneqq \alpha \mathbf{w}_{t,i,s-1}^\top \del_{t,i,s-1}\mathbf{w}_{t,i,s} + \alpha^2 \mathbf{w}_{t,i,s-1}^\top \mathbf{B}_{t,i,s-1}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}$. By expanding $\mathbf{e}_{t,i,s}$, we find

{\color{blue}
\begin{align}
 \mathbf{e}_{t,i,s}   &= \big(\mathbf{I}_d -  \alpha \mathbf{{B}}_{t,i,s-1} \mathbf{B}_{t,i,s-1}^\top + \alpha^2 \langle \mathbf{w}_{t,i,s-1}, \mathbf{B}_{t,i,s-1}^\top\mathbf{e}_{t,i,s-1}\rangle \mathbf{I}_d   - \alpha \| \mathbf{{w}}_{t,i,s-1}\|_2^2 \mathbf{I}_{d} \big)\mathbf{e}_{t,i,s-1} \nonumber \\
    &\quad + \alpha \mathbf{{B}}_{t,i,s-1} \mathbf{B}_{t,i,s-1}^\top (\mathbf{\Sigma}_{t,i,s-1}- \mathbf{I}_d)\mathbf{e}_{t,i,s-1} \nonumber \\
    &\quad - \alpha^2   \langle \mathbf{w}_{t,i,s-1}, \mathbf{B}_{t,i,s-1}^\top\mathbf{e}_{t,i,s-1}\rangle (\mathbf{I}_{d}  - \mathbf{\Sigma}_{t,i,s-1}) \mathbf{e}_{t,i,s-1}  \nonumber \\
    &\quad  -   \alpha^2 \langle \mathbf{w}_{t,i,s-1}, \mathbf{B}_{t,i,s-1}^\top(\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s-1} )\mathbf{e}_{t,i,s-1}\rangle \mathbf{\Sigma}_{t,i,s-1} \mathbf{e}_{t,i,s-1}   \nonumber \\
    &\quad  +  \alpha \| \mathbf{{w}}_{t,i,s-1}\|_2^2 (\mathbf{I}_d - \mathbf{\Sigma}_{t,i,s-1} ) \mathbf{e}_{t,i,s-1} \nonumber \\
    &\quad - \alpha  \mathbf{B}_{t,i,s+1}\mathbf{B}_{t,i,s-1}^\top \tfrac{1}{b}\mathbf{X}_{t,i,s-1}^\top\mathbf{z}_{t,i,s-1} - \alpha  \tfrac{1}{b}\mathbf{X}_{t,i,s-1}^\top\mathbf{z}_{t,i,s-1}\langle\mathbf{w}_{t,i,s-1},\mathbf{w}_{t,i,s+1}\rangle \nonumber \\
    &=  \big(\mathbf{I}_d -  \mathbf{\hat{B}}_{t,i,s-1} \mathbf{\hat{B}}_{t,i,s-1}^\top + \tilde{\del}_{t,i,s-1} + \omega_{t,i,s-1}\mathbf{I}_{d} \big)\mathbf{e}_{t,i,s-1}   + \mathbf{n}_{t,i,s-1} \label{86}
\end{align}
where  $\tilde{\del}_{t,i,s-1} \coloneqq \mathbf{\hat{B}}_{t,i,s-1} \mathbf{\hat{B}}_{t,i,s-1}^\top - \alpha  \mathbf{{B}}_{t,i,s-1} \mathbf{{B}}_{t,i,s-1}^\top $, $\omega_{t,i,s-1}\coloneqq  \alpha^2 \langle \mathbf{w}_{t,i,s-1}, \mathbf{B}_{t,i,s-1}^\top\mathbf{e}_{t,i,s-1}\rangle   - \alpha \| \mathbf{{w}}_{t,i,s-1}\|_2^2$, and $\mathbf{n}_{t,i,s-1}$  contains the finite-sample noise errors and satisfies 
\begin{align}
  \left\| \tfrac{1}{M}\sum_{i=1}^M \mathbf{A} \mathbf{n}_{t,i,s-1} \right\| &\leq c \|\mathbf{A}\| (L_{\max}+ \sigma)\delta 
\end{align}
for an absolute constant $c$ and any fixed matrix $\mathbf{A} \in \mathbb{R}^{k \times d}$ with probability at least $1- $ due to Lemmas \ref{lem:concen1} and . Multiplying both sides of \eqref{86} by $\mathbf{B}_t^\top$ and $\mathbf{w}_{t,i,s}^\top$ and repeating \eqref{86} recursively yields
\begin{align}
    &\tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_t^\top \mathbf{e}_{t,i,s} \mathbf{w}_{t,i,s}^\top  \nonumber \\
    &= \tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_t^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{e}_{t,i,s-1}\mathbf{w}_{t,i,s}^\top  \nonumber \\
    &\quad + \tfrac{1}{M}\sum_{i=1}^M\mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1}  - \omega_{t,i,s-1}\mathbf{I}_d\big) (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\mathbf{w}_{t,i,s}^\top   \nonumber \\
    &\quad + \tfrac{1}{M}\sum_{i=1}^M\mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)\mathbf{e}_{t,i,s-2}\mathbf{w}_{t,i,s}^\top  + \tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_t^\top\mathbf{n}_{t,i,s-1}\mathbf{w}_{t,i,s}^\top  \nonumber \\
    &\quad + \tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big)\mathbf{n}_{t,i,s-2}\mathbf{w}_{t,i,s}^\top \label{3terms2}
\end{align}








% Therefore, averaging over $[M]$, multiplying both sides by $\mathbf{B}_t$ and using Lemmas \ref{lem:concen1} and \ref{}, along with the Cauchy-Schwarz Inequality, we obtain
% \begin{align}
% \tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_t^\top \mathbf{e}_{t,i,s} &=  \tfrac{1}{M}\sum_{i=1}^M\mathbf{B}_{t}^\top   \big(\mathbf{I}_d -  \alpha \mathbf{{B}}_{t,i,s-1} \mathbf{B}_{t,i,s-1}^\top + \alpha^2 \langle \mathbf{w}_{t,i,s-1}, \mathbf{B}_{t,i,s-1}^\top\mathbf{e}_{t,i,s-1}\rangle \mathbf{I}_d   - \alpha \| \mathbf{{w}}_{t,i,s-1}\|_2^2 \mathbf{I}_{d} \big)\mathbf{e}_{t,i,s-1} \nonumber \\
%  &\quad + O( \alpha^{-0.5} (L_{\max}+ \sigma)\delta ) \nonumber \\
%  &=  \tfrac{1}{M}\sum_{i=1}^M\mathbf{B}_{t}^\top   \big(\mathbf{I}_d -  \mathbf{\hat{B}}_{t,i,s-1} \mathbf{\hat{B}}_{t,i,s-1}^\top + \tilde{\del}_{t,i,s-1} + \omega_{t,i,s-1}\mathbf{I}_{d} \big)\mathbf{e}_{t,i,s-1} \nonumber \\
%  &\quad + O( \alpha^{-0.5} (L_{\max}+ \sigma)\delta ) \nonumber \\
% \end{align}
% where $O(\cdot)$ denotes a vector whose Euclidean norm scales as such,  $\tilde{\del}_{t,i,s-1} \coloneqq \mathbf{\hat{B}}_{t,i,s-1} \mathbf{\hat{B}}_{t,i,s-1}^\top - \alpha  \mathbf{{B}}_{t,i,s-1} \mathbf{{B}}_{t,i,s-1}^\top $, and $\omega_{t,i,s-1}\coloneqq  \alpha^2 \langle \mathbf{w}_{t,i,s-1}, \mathbf{B}_{t,i,s-1}^\top\mathbf{e}_{t,i,s-1}\rangle   - \alpha \| \mathbf{{w}}_{t,i,s-1}\|_2^2$






}

% \begin{align}
%     \mathbf{e}_{t,i,s} &= (\mathbf{I}_d - \alpha \mathbf{B}_{t,i,s-1}\mathbf{B}_{t,i,s-1}^\top - \alpha \mathbf{w}_{t,i,s-1}^\top \del_{t,i,s-1}\mathbf{w}_{t,i,s}\mathbf{I}_d - \alpha^2 \mathbf{w}_{t,i,s-1}^\top \mathbf{B}_{t,i,s-1}^\top \mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{I}_d)\mathbf{e}_{t,i,s-1}  \nonumber \\
%     &\quad + noise \nonumber \\
%     &= (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{e}_{t,i,s-1}  + \big( \tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big)\mathbf{e}_{t,i,s-1}  \nonumber \\
%     &= (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{e}_{t,i,s-1}  + \big(\tilde{\del}_{t,i,s-1}  - \omega_{t,i,s-1}\mathbf{I}_d\big) (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}  \nonumber \\
%     &\quad + \big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)\mathbf{e}_{t,i,s-2} 
% \end{align}

% Therefore, 
% \begin{align}
%     \mathbf{B}_t^\top \mathbf{e}_{t,i,s}
%     &= \mathbf{B}_t^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{e}_{t,i,s-1}  + \mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1}  - \omega_{t,i,s-1}\mathbf{I}_d\big) (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}  \nonumber \\
%     &\quad + \mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)\mathbf{e}_{t,i,s-2}  \label{3terms}
% \end{align}

For the first sum, we have
\begin{align}
    & \left\|\tfrac{1}{M}\sum_{i=1}^M \mathbf{B}_t^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{e}_{t,i,s-1}\mathbf{w}_{t,i,s}^\top \right\|_2  \nonumber \\
    &\leq \left\|\tfrac{1}{M}\sum_{i=1}^M\mathbf{B}_{t,i,s-1}^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{e}_{t,i,s-1}\mathbf{w}_{t,i,s}^\top\right\|_2\nonumber \\
    &\quad + \left\|\tfrac{1}{M}\sum_{i=1}^M(\mathbf{B}_t - \mathbf{B}_{t,i,s-1})^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{e}_{t,i,s-1}\mathbf{w}_{t,i,s}^\top\right\|_2 \nonumber \\
    &= \left\|\tfrac{1}{M}\sum_{i=1}^M(\mathbf{B}_t - \mathbf{B}_{t,i,s-1})^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top\right\|  \nonumber \\
    &\leq \alpha^{0.5} L_{\max}^2 \tfrac{1}{M}\sum_{i=1}^M  \nonumber \\
    &---- \nonumber \\
    &= \left\|\tfrac{1}{M}\sum_{i=1}^M \sum_{r=1}^{s-1} (\mathbf{B}_{t,i,r-1} - \mathbf{B}_{t,i,r} )^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{B}_{\ast}\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top\right\|_2  \nonumber \\
    &\leq \sum_{r=1}^{s-1} \left\|\tfrac{1}{M}\sum_{i=1}^M (\mathbf{B}_{t,i,r-1} - \mathbf{B}_{t,i,r} )^\top(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{B}_\ast\mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top\right\|_2  \nonumber \\
    &\leq c \max_{i \in [M]}\| (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{B}_\ast \mathbf{w}_{\ast,t,i}\mathbf{w}_{t,i,s}^\top\|_2  \alpha^{1.5} \tau L_{\max}( L_{\max}+ (L_{\max}+\sigma)\delta)  \nonumber \\
    &\leq c\alpha^{2} \tau L_{\max}^2( L_{\max}+ \sigma\delta)   \dist_t \nonumber
\end{align}
using that $\|(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-1}\mathbf{\hat{B}}_{t,i,s-1}^\top)\mathbf{B}_\ast\|= \dist(\mathbf{B}_{t,i,s}, \mathbf{B}_\ast) \leq 2\dist_t$ by $A_3(t,i,\tau-1)$.
For the second term in \eqref{3terms}, we have
\begin{align}
   \| \mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1}  - \omega_{t,i,s-1}\mathbf{I}_d\big) &(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2 \nonumber \\
   &\leq  \| \mathbf{B}_t^\top \tilde{\del}_{t,i,s-1}  (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2   \nonumber \\
    &\quad + |\omega_{t,i,s-1} |\| \mathbf{B}_t^\top (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2    \nonumber \\
    &\leq  \| \mathbf{B}_t^\top \tilde{\del}_{t,i,s-1}  (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2   \nonumber \\
    &\quad + c \alpha^{1.5} L_{\max}^3 \dist_t  
\end{align}
and
\begin{align}
    \| &\mathbf{B}_t^\top \tilde{\del}_{t,i,s-1}  (\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2 \nonumber\\
    &\leq \| \mathbf{B}_t^\top \mathbf{\hat{B}}_{t,i,s-1}   \mathbf{\hat{B}}_{t,i,s-1}^\top(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2  \nonumber \\
    &\quad + \alpha\| \mathbf{B}_t^\top \mathbf{{B}}_{t,i,s-1}   \mathbf{{B}}_{t,i,s-1}^\top(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2  \nonumber \\
    &\leq \| \mathbf{B}_t^\top \mathbf{\hat{B}}_{t,i,s-1} (\mathbf{R}^{-1}_{t,i,s-1})^\top  \mathbf{{B}}_{t,i,s-1}^\top(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2  \nonumber \\
    &\quad + \alpha\| \mathbf{B}_t^\top \mathbf{{B}}_{t,i,s-1}   \mathbf{{B}}_{t,i,s-1}^\top(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2  \nonumber \\
    &\leq \alpha \| \mathbf{B}_t^\top \mathbf{\hat{B}}_{t,i,s-1} (\mathbf{R}^{-1}_{t,i,s-1})^\top  \mathbf{{w}}_{t,i,s-2} \mathbf{e}_{t,i,s-2}^\top(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2  \nonumber\\
    &\quad \alpha^2\| \mathbf{B}_t^\top \mathbf{{B}}_{t,i,s-1} \mathbf{{w}}_{t,i,s-2}  \mathbf{{e}}_{t,i,s-2}^\top(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top)\mathbf{e}_{t,i,s-2}\|_2 \nonumber \\
    &\leq c\alpha^{1.5} L_{\max}^3 \dist_t^2
\end{align}
using that $\mathbf{B}_{t,i,s-2}(\mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-2}\mathbf{\hat{B}}_{t,i,s-2}^\top) = \mathbf{0}$. For the third term in \eqref{3terms}, for any $s>2$,
\begin{align}
    \| &\mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)\mathbf{e}_{t,i,s-2}  \|_2 \nonumber \\
    &\leq  \| \mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)( \tilde{\del}_{t,i,s-3}  - \omega_{t,i,s-3}\mathbf{I}_d)\mathbf{e}_{t,i,s-3} \|_2\nonumber \\
    &\quad + \|\mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)( \mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-3}\mathbf{\hat{B}}_{t,i,s-3}^\top)\mathbf{e}_{t,i,s-3} \|_2  \nonumber \\
    &\leq  \| \mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)( \tilde{\del}_{t,i,s-3}  - \omega_{t,i,s-3}\mathbf{I}_d)\mathbf{e}_{t,i,s-3} \|_2 \nonumber \\
    &\quad + c \alpha^{3.5} \tau^2 c_{\del}^2 L_{\max} \dist_t  \nonumber \\
    &\vdots \nonumber \\
    &\leq \bigg\|\mathbf{B}_t^\top\prod_{r=1}^s\big(\tilde{\del}_{t,i,s-r} - \omega_{t,i,s-r}\mathbf{I}_d\big) \mathbf{e}_{t}\bigg\|_2  + c \alpha^{3.5}\tau^2 c_{\del}^2 L_{\max}\dist_t \sum_{r=0}^s \alpha^{2r} \tau^r c_{\del}^r \nonumber \\
    &\leq  \bigg\|\mathbf{B}_t^\top\prod_{r=1}^s\big(\tilde{\del}_{t,i,s-r} - \omega_{t,i,s-r}\mathbf{I}_d\big) \mathbf{e}_{t}\bigg\|_2  + \frac{c \alpha^{3.5}\tau^2 c_{\del}^2  L_{\max} \dist_t}{1 - \alpha^{2} \tau c_{\del} L_{\max}}  \nonumber  \\
    % c \alpha^{3.5} \tau^2 c_{\del}^2 L_{\max}
    &\leq  c \alpha^{2s - 0.5} \tau^{s} c_{\del}^s L_{\max} + {c' \alpha^{3.5}\tau^2 c_{\del}^2  L_{\max} \dist_t} \nonumber
\end{align}


----




For the third term in \eqref{3terms}, for any $s>2$,
\begin{align}
    \| &\mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)\mathbf{e}_{t,i,s-2}  \|_2 \nonumber \\
    &\leq  \| \mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)( \tilde{\del}_{t,i,s-3}  - \omega_{t,i,s-3}\mathbf{I}_d)\mathbf{e}_{t,i,s-3} \|_2\nonumber \\
    &\quad + \|\mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)( \mathbf{I}_d - \mathbf{\hat{B}}_{t,i,s-3}\mathbf{\hat{B}}_{t,i,s-3}^\top)\mathbf{e}_{t,i,s-3} \|_2  \nonumber \\
    &\leq  \| \mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)( \tilde{\del}_{t,i,s-3}  - \omega_{t,i,s-3}\mathbf{I}_d)\mathbf{e}_{t,i,s-3} \|_2 \nonumber \\
    &\quad + c \alpha^{3.5} \tau^2 c_{\del}^2 L_{\max} \dist_t {\color{blue} \times (1 + \tfrac{\sqrt{k}}{\dist_t \sqrt{b}}) } \nonumber \\
    &\vdots \nonumber \\
    &\leq \bigg\|\mathbf{B}_t^\top\prod_{r=1}^s\big(\tilde{\del}_{t,i,s-r} - \omega_{t,i,s-r}\mathbf{I}_d\big) \mathbf{e}_{t}\bigg\|_2  + c \alpha^{3.5}\tau^2 c_{\del}^2 L_{\max}\dist_t \sum_{r=0}^s \alpha^{2r} \tau^r c_{\del}^r \nonumber \\
    &\leq  \bigg\|\mathbf{B}_t^\top\prod_{r=1}^s\big(\tilde{\del}_{t,i,s-r} - \omega_{t,i,s-r}\mathbf{I}_d\big) \mathbf{e}_{t}\bigg\|_2  + \frac{c \alpha^{3.5}\tau^2 c_{\del}^2  L_{\max} \dist_t}{1 - \alpha^{2} \tau c_{\del} L_{\max}}  \nonumber  \\
    % c \alpha^{3.5} \tau^2 c_{\del}^2 L_{\max}
    &\leq  c \alpha^{2s - 0.5} \tau^{s} c_{\del}^s L_{\max} {\color{blue} (1 + \tfrac{\sqrt{k}}{\sqrt{b}})^{s}} + \frac{c \alpha^{3.5}\tau^2 c_{\del}^2  L_{\max}^3 \dist_t}{1 - \alpha^{2} \tau c_{\del} L_{\max}^3 } {\color{blue}  + \frac{c \alpha^{3.5}\tau^2 c_{\del}^2  L_{\max}^3 }{1 - \alpha^{2} \tau c_{\del} L_{\max}^3 }  \frac{\sqrt{k}}{\sqrt{b}} } \nonumber 
\end{align}
and for $s=2$ we have
\begin{align}
    \| &\mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)\mathbf{e}_{t,i,s-2}  \|_2 
    &\leq  c \alpha^{2s - 0.5} \tau^{s} c_{\del}^s L_{\max}  \nonumber 
\end{align}
% which is fine.

Need to show that distance doesn't decrease locally. (done, just move it up)

{\color{blue} for FS, these arguments are fine. do not need to deal with higher-order products, just use cauchy schwarz.
$(1+ \tfrac{\sqrt{k}}{\sqrt{b}})^s$ is not a problem because we can just make $\alpha$ smaller

% problem is that we will get

$\alpha^6 \tau^3 \tfrac{\sqrt{k}}{\sqrt{b}} $ term (from all 3 terms above), thus need $\alpha^6 \tau^3 \tfrac{\sqrt{k}}{\sqrt{b}} \leq  \alpha^4 \tau \equiv b \geq \alpha^4 \tau^4 k $ which is satisfied by $b \geq  \tau^2 k $ or $\alpha$ is smaller

-- note: can replce b with Mb by averaging over users

but can we get control of projected distnace? we should be able to. will need Mb > tau2 though... but we can intuitively justify this


also remember that deldtilde + omega term no longer sales w alpha2 tau




fr the distance term, we will also get a 
$ \sqrt{d}/\sqrt{N \tau} $ term (in fresh samples case)


is the noise term even ok?


}



----


and for $s=2$ we have
\begin{align}
    \| &\mathbf{B}_t^\top\big(\tilde{\del}_{t,i,s-1} - \omega_{t,i,s-1}\mathbf{I}_d\big) \big(\tilde{\del}_{t,i,s-2}  - \omega_{t,i,s-2}\mathbf{I}_d\big)\mathbf{e}_{t,i,s-2}  \|_2 
    \leq  c \alpha^{2s - 0.5} \tau^{s} c_{\del}^s L_{\max}  \nonumber 
\end{align}
% which is fine.
Thus, using $\|\mathbf{w}_{t,i,s}\|_2\leq c \sqrt{\alpha}L_{\max}$, we have
\begin{align}
  \|  \alpha^2 \mathbf{E}_4 \|_2 &\leq c \alpha^{2.5} L_{\max} \sum_{s=2}^\tau (\alpha^{2s-0.5}\tau^s c_{\del}^s L_{\max} + \alpha^{3.5} \tau^2 c_{\del}^2 L_{\max}\dist_t  +  \alpha^{1.5} L_{\max}^3 \dist_t^2 )\nonumber \\
  &\leq c\alpha^{6}\tau^{2} c_{\del}^2L_{\max}^2 + c (\alpha^{6} \tau^3 c_{\del}^2 L_{\max}^2   + \alpha^{4} \tau L_{\max}^4 )\dist_t \nonumber
\end{align}



The noise terms are bounded as 
\begin{align}
    
\end{align}

% Now, noting that $\|\mathbf{B}_{\ast,t,\perp}\|_2\leq \dist_t$, we have
% \begin{align}
%      \|\alpha^2\mathbf{E}_4\|_2 &= \alpha^2\left\| \mathbf{B}_t^\top\tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} \mathbf{e}_{t,i,s}\mathbf{w}_{t,i,s}^\top \right\|_2 \nonumber \\
%      &=\alpha^2\left\| \mathbf{B}_t^\top\tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} (\mathbf{I}_d - )\mathbf{e}_{t,i,s-1}\mathbf{w}_{t,i,s}^\top \right\|_2 \nonumber \\
%      &\leq   \nonumber 
%     %  &\leq \alpha^2 \sum_{s=2}^{\tau-1} (\alpha^2 \tau^x c_{\del})^{s-1} + \alpha^2 \left\|\tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} \mathbf{B}_t^\top \deld_{t,i,s-1}\dots\deld_{t,i,1}\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i,s}^\top \right\|_2 \nonumber \\
%     %  &\leq \alpha^2 \sum_{s=2}^{\tau-1} (\alpha^2 \tau^x c_{\del})^{s-1} + \alpha^2 \left\| \tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} \mathbf{B}_{t,i,s-1}^\top \deld_{t,i,s-1}\dots\deld_{t,i,1}\mathbf{B}_{\ast,t,\perp}\mathbf{w}_{\ast,t,i} \mathbf{w}_{t,i,s}^\top \right\|_2 + \alpha^4 \tau^2 \dist_t L_{\max}^4 \nonumber \\
%     %  &\leq \alpha^2 \sum_{s=2}^{\tau-1} (\alpha^2 \tau^x c_{\del})^{s-1} + \alpha^4\tau^{1+x} L_{\max}^2 c_{\del}\dist_t + \alpha^4 \tau^2 \dist_t L_{\max}^4 \nonumber \\
%     %  &\leq c \alpha^4 \tau^x c_{\del}  + \alpha^4 \tau L_{\max}^2 ( \tau L_{\max}^2 + \tau^x c_{\del}) \dist_t 
% \end{align}
% Thus, we can get $x= 1-\epsilon$ if $\dist_t$ converges at rate $\alpha^2 \tau^{1+\epsilon}$. We know that larger $\tau$ improves the condition number in the convergence of $\dist_t$.  $\tau^2$ term is unavoidable.

Combining all terms, we obtain
\begin{align}
    \|\del_{t+1}\|_2 &\leq (1 - \alpha^2 E_0 \tilde{\mu}^2_\ast )\|\del_t\|_2 + c\alpha^{6}\tau^{2} c_{\del}^2L_{\max}^2 + c \alpha^4 L_{\max}^4  + c (\alpha^{6} \tau^3 c_{\del}^2 L_{\max}^2   + \alpha^{4} \tau L_{\max}^4 )\dist_t \nonumber \\
    &\quad + {\color{blue} \alpha^4 L^4 +  2\alpha^2 L (L+\sigma) \delta + 2 \alpha^4 \tau L^4 + 5\alpha^2 L^2 \|\del_t\|^2  + \alpha^2 \tau L(L+\sigma)\delta} \nonumber \\
    &\quad {\color{blue}\rightarrow + 2 \alpha^4 \tau L^4 + 5\alpha^2 L^2 \|\del_t\|^2  + \alpha^2 \tau L(L+\sigma)\delta  }
    &\quad  \vdots \nonumber \\
    &\leq (1 - \alpha^2 E_0 \tilde{\mu}^2_\ast )^t\|\del_0\|_2 \nonumber \\
    &\quad + \sum_{t' = 1}^t (1 - \alpha^2 E_0 \tilde{\mu}_\ast^2)^{t-t'} (c\alpha^{6}\tau^{2} c_{\del}^2L_{\max}^2 + c \alpha^4 L_{\max}^4  + c (\alpha^{6} \tau^3 c_{\del}^2 L_{\max}^2   + \alpha^{4} \tau L_{\max}^4 )\dist_{t'})  \nonumber \\ 
      &\leq \|\del_0\|_2 + c \alpha^4 \tau^2 c_{\del}^2 (\tfrac{L_{\max}^2}{\tilde{\mu}_\ast^2}+ \tfrac{L_{\max}^2}{{\mu}_\ast^2}) +  c \alpha^2 L_{\max}^2 ( \tfrac{L_{\max}^2}{\tilde{\mu}_\ast^2} + \tfrac{L_{\max}^2}{\mu_\ast^2} )\nonumber \\
      &\leq c\alpha^2 \tau c_{\del}
    % &\leq \alpha^2 \tau c_{\del} -  \alpha^4 \tau c_{\del} E_0 \tilde{\mu}^2_\ast 
\end{align}
Choose $c_{\del} = c L_{\max}^2 ( \tfrac{L_{\max}^2}{\tilde{\mu}_\ast^2} + \tfrac{L_{\max}^2}{\mu_\ast^2} )$.

will need to get rid of a tau via more samples

can tighten the alpha6 tau3 term

but still we have the initial noise






\end{proof}


==> a2tau_geq_1.tex <==


\section{Meeting 4/8}

Still cannot complete the proof when $\alpha^2 \tau \gtrsim 1$...

Notations:
\begin{align}
\hat{\mu}_{\ast}^2 &= \sigma_{\min}\left(\tfrac{1}{n}\sum_{i=1}^n \frac{1}{\|\mathbf{w}_{\ast,i} \|_2^2}\mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \right) \nonumber \\
\bar{\mathbf{w}}_{\ast} &= \tfrac{1}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i} \nonumber \\
    \bar{\mu}_\ast^2 &= \sigma_{\min}\left(\tfrac{1}{n}\sum_{i=1}^n (\mathbf{w}_{\ast,i} - \bar{\mathbf{w}}_{\ast}  )(\mathbf{w}_{\ast,i} - \bar{\mathbf{w}}_{\ast}  )^\top \right) \nonumber
\end{align}

Two difficulties:

\begin{enumerate}
    \item Cannot show that the distance is converging: we have
    \begin{align}
        \mathbf{B}_{t+1} &= \mathbf{B}_t\left(\tfrac{1}{n}\sum_{i=1}^n \prod_{s=1}^\tau (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top ) \right) + \mathbf{B}_\ast \left(\tfrac{\alpha}{n}\sum_{i=1}^n \mathbf{w}_{\ast,i}\sum_{s=1}^\tau\mathbf{w}_{t,i,s}^\top\prod_{r=s}^{\tau}(\mathbf{I}- \alpha\mathbf{w}_{t,i,r}\mathbf{w}_{t,i,r}^\top) \right) \nonumber \\
       \| \mathbf{B}_{\ast,\perp}^\top\mathbf{B}_{t+1}\|_2 &= \|\mathbf{B}_{\ast,\perp}^\top\mathbf{B}_t\|_2\left\|\tfrac{1}{n}\sum_{i=1}^n \prod_{s=1}^\tau (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top ) \right\|_2 \nonumber 
    \end{align}
    Empirically, 
    \begin{align}
        \left\|\tfrac{1}{n}\sum_{i=1}^n \prod_{s=1}^\tau (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top ) \right\|_2 &\approx 1 - \alpha \sigma_{\min}^2(\mathbf{B}_\ast^\top \mathbf{B}_t) \hat{\mu}_\ast^2 \label{recov}
    \end{align}
    this approximation is tight when $\alpha \sigma_{\min}^2(\mathbf{B}_\ast^\top \mathbf{B}_t) \hat{\mu}_\ast^2 \ll 1$ (note that this quantity scales independently of $\alpha$). If we assume that {\color{red}
    \begin{align}
        \prod_{s=1}^\tau (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top ) \approx  (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,\tau}\mathbf{w}_{t,i,\tau}^\top )^\tau \label{54}
    \end{align}}
    and $\mathbf{w}_{t,i,\tau}\approx \alpha \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i}$, then we recover \eqref{recov} since
    \begin{align}
        \left\|\tfrac{1}{n}\sum_{i=1}^n \prod_{s=1}^\tau (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,s}\mathbf{w}_{t,i,s}^\top ) \right\|_2 &\approx \left\|\tfrac{1}{n}\sum_{i=1}^n (\mathbf{I}_k - \alpha \mathbf{w}_{t,i,\tau}\mathbf{w}_{t,i,\tau}^\top  )^\tau \right\|_2 \nonumber \\
       &\approx \left\|\tfrac{1}{n}\sum_{i=1}^n (\mathbf{I}_k - \alpha^3 \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{B}_\ast^\top  \mathbf{B}_t )^\tau \right\|_2 \nonumber \\
        &= \left\| \mathbf{I}_k - \tfrac{1}{n}\sum_{i=1}^n\frac{1}{\| \mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i}\|_2^2}\mathbf{B}_t^\top \mathbf{B}_\ast \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top \mathbf{B}_\ast^\top  \mathbf{B}_t  \right\|_2 \nonumber \\
        &\leq  \left\| \mathbf{I}_k -\alpha^2{\sigma_{\min}^2(\mathbf{B}_t^\top \mathbf{B}_\ast)} \sigma_{\min}(\tfrac{1}{n}\sum_{i=1}^n\frac{1}{\| \mathbf{w}_{\ast,i}\|_2^2} \mathbf{w}_{\ast,i}\mathbf{w}_{\ast,i}^\top)  \right\|_2 \nonumber \\
        &\leq 1 - \alpha^2 \sigma_{\min}^2(\mathbf{B}_\ast^\top \mathbf{B}_t) \hat{\mu}_\ast^2 
    \end{align}
    The difficulty is in showing that \eqref{54} holds. 
    
    Assume $\alpha \sigma_{\min}^2(\mathbf{B}_\ast^\top \mathbf{B}_t) = 0.5$. Then, since \eqref{54} is tight when $\hat{\mu}_\ast^2$ is small, the error in the approximation in \eqref{54} must scale with something smaller than $\hat{\mu}_\ast^2$. Empirically, it scales with $\alpha^4 \hat{\mu}_\ast^2 \ll \hat{\mu}_\ast^2 $. However, we are only  able to upper bound the error by a constant. Approaches we have tried:
    \begin{itemize}
        \item \textbf{Simply use the fast convergence of $\mathbf{w}_{t,i,s}$.}
        Let $\|\mathbf{I}_k - \alpha \mathbf{B}_{t,i,s}^\top  \mathbf{B}_{t,i,s} \|_2 \leq D$ for all $s$ (we can show this is true if $\|\mathbf{I}_k - \alpha \mathbf{B}_{t}^\top  \mathbf{B}_{t} \|_2 = O(D)$). Then we can show:
        \begin{align}
            \|\mathbf{w}_{t,i,s+1}- \mathbf{w}_{t,i,s}\|_2 &\leq \sqrt{\alpha} D^s + \alpha^{2.5} (1 - \alpha^2 \|\mathbf{w}_{\ast,i}\|_2^2 )^{2s} \| \mathbf{B}_{t}\mathbf{w}_{t} - \mathbf{B}_{\ast} \mathbf{w}_{\ast,i}\|_2^2
        \end{align}
        This implies that 
        \begin{align}
            \|\mathbf{w}_{t,i,\tau}- \mathbf{w}_{t,i,s}\|_2 &\leq \sqrt{\alpha} \sum_{r=s}^\tau D^r + \alpha^{2.5} \| \mathbf{B}_{t}\mathbf{w}_{t} - \mathbf{B}_{\ast} \mathbf{w}_{\ast,i}\|_2^2 \sum_{r=s}^\tau (1 - \alpha^2 \|\mathbf{w}_{\ast,i}\|_2^2 )^{2r} \nonumber \\
            &\lesssim \sqrt{\alpha} \frac{ D^s}{1 - D} + 0.5 \sqrt{\alpha} (1 - \alpha^2 \|\mathbf{w}_{\ast,i}\|_2^2 )^{2s}\label{55}
        \end{align}
        
        Now make two-stage argument:
        
        Let $\mathbf{w}_s = \mathbf{w}_{t,i,s}$ and  $\boldsymbol{\delta}_s \coloneqq \mathbf{I}_k - \alpha \mathbf{w}_{s}\mathbf{w}_{s}^\top$.
        
        \begin{align}
            \prod_{s=1}^\tau \boldsymbol{\delta}_s - \boldsymbol{\delta}_\tau^\tau = (\prod_{s=1}^{\tau'} \boldsymbol{\delta}_s) (\prod_{z=\tau'}^{\tau} \boldsymbol{\delta}_z - \boldsymbol{\delta}_\tau^{\tau-\tau'}) + \prod_{s=1}^{\tau'} (\boldsymbol{\delta}_s - \boldsymbol{\delta}_\tau^{\tau'})\boldsymbol{\delta}_\tau^{\tau - \tau'}
        \end{align}
        for some $\tau' : \alpha^2 \tau' \ll 1$.
        We know: 
        \begin{align}
            \| \prod_{s=1}^{\tau'} (\boldsymbol{\delta}_s - \boldsymbol{\delta}_\tau^{\tau'})\|_2 &\leq \sum_{s = 1}^{\tau'} \alpha\|\mathbf{w}_{s}\mathbf{w}_{s}^\top -  \mathbf{w}_{\tau}\mathbf{w}_{\tau}^\top\| + \sum_{s = 1}^{\tau'}\sum_{s' = 1}^{\tau'} \alpha^2\|\mathbf{w}_{s}\mathbf{w}_{s}^\top -  \mathbf{w}_{\tau}\mathbf{w}_{\tau}^\top\|\|\mathbf{w}_{s'}\mathbf{w}_{s'}^\top -  \mathbf{w}_{\tau}\mathbf{w}_{\tau}^\top\| + \dots \nonumber \\
            &\leq \alpha^2 \tau' + \alpha^4 (\tau')^2 + \dots \nonumber \\
            &= c\alpha^2 \tau'
        \end{align}
        Meanwhile, using \eqref{55} and assuming $D < (1 - \alpha^2 \|\mathbf{w}_{\ast,i}\|_2^2)$, we can show 
        \begin{align}
           \left \| \prod_{z=\tau'}^{\tau} (\boldsymbol{\delta}_z - \boldsymbol{\delta}_\tau^{\tau-\tau'})\right\|_2 &\leq (1 - \alpha^2 \|\mathbf{w}_{\ast,i}\|_2^2)^{2\tau'}
        \end{align}
        
        So
        \begin{align}
          \left  \|(\prod_{s=1}^{\tau'} \boldsymbol{\delta}_s) (\prod_{z=\tau'}^{\tau} \boldsymbol{\delta}_z - \boldsymbol{\delta}_\tau^{\tau-\tau'}) + \prod_{s=1}^{\tau'} (\boldsymbol{\delta}_s - \boldsymbol{\delta}_\tau^{\tau'})\boldsymbol{\delta}_\tau^{\tau - \tau'}\right\|_2 &\leq c \alpha^2 \tau' + (1 - \alpha^2 \|\mathbf{w}_{\ast,i}\|_2^2)^{2\tau'}
        \end{align}
        but there is no $\tau'$ such that the RHS is small (i.e. $O(\alpha^2)$)
        
        \item \textbf{Recursive approach.} Let 
        \begin{align}
            \mathbf{E}_s &\coloneqq  \prod_{r=1}^s \boldsymbol{\delta}_r -  \boldsymbol{\delta}_s^s
        \end{align}
        and note that our goal is to control $\|\mathbf{E}_\tau\|_2$. We have:
        \begin{align}
            \mathbf{E}_{s+1} &=  \prod_{r=1}^{s+1} \boldsymbol{\delta}_r -  \boldsymbol{\delta}_{s+1}^{s+1} \nonumber \\
            &= (\prod_{r=1}^{s} \boldsymbol{\delta}_r -  \boldsymbol{\delta}_{s}^{s})\boldsymbol{\delta}_{s+1}  \nonumber \\
            &\quad +(\boldsymbol{\delta}_s^s -  \boldsymbol{\delta}_{s+1}^{s})\boldsymbol{\delta}_{s+1} \nonumber \\
            &= \mathbf{E}_s\boldsymbol{\delta}_{s+1}  +(\boldsymbol{\delta}_s^s -  \boldsymbol{\delta}_{s+1}^{s})\boldsymbol{\delta}_{s+1}
        \end{align}
        from which we can show
        \begin{align}
            \|\mathbf{E}_{s+1}\|_2 &\leq \|\mathbf{E}_s\boldsymbol{\delta}_{s+1}\|_2  +\|(\boldsymbol{\delta}_s^s -  \boldsymbol{\delta}_{s+1}^{s})\boldsymbol{\delta}_{s+1}\|_2 \nonumber \\
            &\leq \|\mathbf{E}_s\|_2  +\|\boldsymbol{\delta}_s^s -  \boldsymbol{\delta}_{s+1}^{s}\|_2 \label{loose?} \\
            &\leq \|\mathbf{E}_s\|_2  +c\alpha^2 (1 - \alpha^2 \|\mathbf{w}_{\ast,i}\|_2^2)^{2s}  \nonumber 
        \end{align}
        which implies $\|\mathbf{E}_\tau\|_2\leq c$, which is not good enough.
        
        There may be looseness in \eqref{loose?} because it ignores the fact that multiplication by $\boldsymbol{\delta}_{s+1}$ causes contraction in exactly one direction ($\mathbf{w}_{s+1}$). However, for this to be useful we must show that most of the energy in $\mathbf{E}_s$ is concentrated in the direction $\mathbf{w}_{s+1}$. But I have not been able to show this...
        
        
        \item Other approaches: 
        
        - Instead of trying to bound the error for each client separately, consider the average error over all clients. But averaging does not seem to give any benefit.
        
        - 

    \end{itemize}
    
    \item $\|\del_t\|_{t+1}\leq \kappa_\ast^{-1}$ 
    
    Recall $\del_{t} \coloneqq \mathbf{I}_k - \alpha\mathbf{B}_t^\top \mathbf{B}_t$ and:
    \begin{align}
  \|\del_{t+1}\|_2 &\leq \underbrace{(1 - \alpha^2 \tilde{\mu}_{\ast}^2)\|\del_t\|_2}_{\text{contraction due to first two local updates}}  + \underbrace{\alpha^2 L_{\max}^2 \|\del_t\|_2^2}_{\text{perturbation due to first two local updates}} \nonumber \\
  &\quad + {\color{red}\alpha^2\underbrace{\bigg\|\mathbf{B}_t^\top\tfrac{1}{n}\sum_{i=1}^n \sum_{s = 2}^{\tau-1} (\mathbf{B}_{t,i,s}\mathbf{w}_{t,i,s}- \mathbf{B}_\ast\mathbf{w}_{\ast,t,i})\mathbf{w}_{t,i,s}^\top\bigg\|_2}_{\text{perturbation due to local updates $>2$}}}
\end{align}
When $\alpha^2 \tau \gtrsim 1$ we do not know to bound the perturbation due to more than 2 local updates. Currently we have that this term is upper bounded by $\dist_t^2$, which means
\begin{align}
        \|\del_{t+1}\|_2 \leq \sum_{s=1}^t(1 - \alpha^2 \bar{\mu}_\ast^2)^{t-s}
        \dist_s^2
    \end{align}
But even if $\dist_s$ is linearly converging, this bound is not tight enough to show $\|\del_t\|_{t+1}\leq \kappa_\ast^{-1}$ (the looseness is in the bound of $\dist_t^2$ on the perturbation term).
\end{enumerate}



